PerfGen: Automated Performance Benchmark Generation for Big Data Analytics

Many symptoms of poor performance in big data analytics such as computational skews, data skews, and memory skews are input dependent. However, due to the lack of inputs that can trigger such performance symptoms, it is hard to debug and test big data analytics. We design PerfGen to automatically generate inputs for the purpose of performance testing. PerfGen overcomes three challenges when naively using automated fuzz testing for the purpose of performance testing. First, typical greybox fuzzing relies on coverage as a guidance signal and thus is unlikely to trigger interesting performance behavior. Therefore, PerfGen provides performance monitor templates that a user can extend to serve as a set of guidance metrics for grey-box fuzzing. Second, performance symptoms may occur at an intermediate or later stage of a big data analytics pipeline. Thus, PerfGen uses a phased fuzzing approach. This approach identifies symptom-causing intermediate inputs at an intermediate stage first and then converts them to the inputs at the beginning of the program with a pseudo-inverse function generated by a large language model. Third, PerfGen defines sets of skew-inspired input mutations, which increases the chance of inducing performance problems. We evaluate PerfGen using four case studies. PerfGen achieves at least 11x speedup compared to a traditional fuzzing approach when generating inputs to trigger performance symptoms. Additionally, identifying intermediate inputs first and then converting them to original inputs enables PerfGen to generate such workloads in less than 0.004% of the iterations required by a baseline approach.

==> asplos_outdated/approach_asplos.tex <==

\begin{figure*}[t]
\centering
   \scalebox{0.95}{\begin{minipage}{0.42\textwidth}
    \begin{subfigure}[t]{1\textwidth}
        \input{code/code_collatz_sparkrdd}
        \caption{A DISC Application \codefont{Collatz.scala}}
            \label{fig:collatz_sparkrdd}
    \end{subfigure}
    \end{minipage}}  
    %\hfill
    \scalebox{0.95}{\begin{minipage}{0.58\textwidth}
    \begin{subfigure}[t]{1\textwidth}
        %\vspace{-1ex}
        \input{code/code_collatz_hybridrdd}
        \vspace{-2ex}
        \caption{Transformed \codefont{Collatz} with \codefont{HybridRDD}}
            \label{fig:collatz_hybridrdd}
            
        \begin{tikzpicture}[overlay]
          \draw[orange,thick,rounded corners] (7.6,2.0) rectangle (10.5,2.5) node[pos=.5] {\textcolor{black}{\bf\footnotesize User-defined function}};
        \end{tikzpicture}
    \end{subfigure}
    \end{minipage}} 
\vspace{-2ex}
\caption{\tool extends Spark's RDD API with \textit{HybridRDD} to support extraction and reuse of individual UDFs without significant program rewriting. While optional, variable types in \ref{fig:collatz_hybridrdd} are shown to highlight type differences.
% \tool isolates the target UDF leveraging source-to-source transformations based on \codefont{HybridRDD} which tracks the RDD transformations. Although Scala does not require explicit types to be declared, variable types are shown in order to highlight type differences as well as input and output data types. \todo{Rewrite caption and references to indicate Collatz program and demonstration of program rewrite}.
}

\end{figure*}


\section{Approach}
Figure~\ref{fig:overview} outlines \tool's phased fuzzing approach for generating an input to reproduce a target performance skew symptom. \tool takes as input a DISC application built on Apache Spark, a target UDF (user-defined function) within that program, an initial program input seed, and a target symptom to reproduce, defined by a monitor template and metric. 

\tool extends a traditional fuzzing workflow with four novel contributions. Section~\ref{sec:udfisolation} describes   
\tool's \textit{HybridRDD} extension to the Spark RDD API in order to support execution of individual UDFs for more precise fuzzing.
Section~\ref{sec:perffeedback} enables a user to specify a desired symptom via execution \textit{metrics} and predefined \textit{monitor templates} which define patterns to detect symptoms. Section~\ref{sec:mutation} leverages schema knowledge from the isolated UDF as well as the symptom definition to define a weighted set of {\it skew-inspired mutations} designed to generate syntactically valid inputs geared towards producing the target skew symptom. Finally, Section~\ref{sec:phasedfuzzing} combines these techniques to fuzz the specified UDF for symptom-reproducing UDF inputs, then leverages an inverse function to derive program inputs which are then used as an enhanced starting point for fuzzing the original 
program from end to end.


% \subsection{UDF Isolation}
\subsection{Targeting UDFs}
\label{sec:udfisolation}
DISC applications inherently have longer latency than other applications, making them unsuitable for iterative fuzz testing~\cite{zhang2020:bigfuzz} which expects millions of invocations per second. Reproducing a specified performance skew is also an extremely rare event to trigger by chance via input mutation, particularly when the symptom occurs deep in the program where mutations are unlikely to result in significant changes.
%Especially when the symptom happens in a later computation stage, the likelihood of reaching the deeper execution path and triggering a specific performance skew by chance becomes lower, as this is similar to finding a specific needle in the midst of very large input space. \todo{edit: either needle in a haystack or remove needle}

To overcome this challenge of test input exploration time while reproducing performance skews, \tool designs a novel phased fuzzing process based on the observation that fuzzing is easier for a single UDF in isolation than fuzzing an entire application  to reach a specific, deep execution path. 
To enable this, \tool requires users to specify a target UDF for analysis (Figure \ref{fig:overview} label 1). However, existing DISC systems such as Spark define datasets in terms of transformations (including UDFs) directly applied to previous datasets. As a result, such programs do not support decoupling UDFs from input datasets without manual refactoring.

In order to automatically extract UDFs from a Spark program, \tool extends the Spark RDD API with its own \textit{HybridRDD} which internally separates transformations from the datasets on which they are applied and stores information about the corresponding input and output data types. In doing so, developers can specify individual \textit{HybridRDD} instances which \tool can then be used to execute their corresponding UDFs without any additional refactoring. Furthermore, the captured input and output data type information can be used in Section \ref{sec:mutation} to define type-compatible mutations for the targeted UDF.

% \tool provides users with a \textit{HybridRDD} API for isolating and extracting individual UDFs from the entire Spark program. 
%\jason{I cut off the last sentence of the original phased fuzzing intro, but left the remainder as it can still be applied to UDF isolation}. 

% \noindent\textbf{Step 1. UDF Isolation.}
%1. clarify that a UDF location is given by a user . 
%You may want to start with the performance symptom, since its \textcolor{red}{error message} is often associated with the UDF location or name  ====> %\qian{starting with error messages is infeasible for performance symptoms}


%When an application shows a sign of poor performance, its symptom (such as an increase in general CPU time, garbage collection time, etc.) is often associated with a particular UDF with intermediate RDDs. Suppose that Bob writes an scientific application 
Figures \ref{fig:collatz_sparkrdd} and \ref{fig:collatz_hybridrdd} illustrate the API changes required to leverage \tool's \textit{HybridRDD} extension for the \CollatzProgramName program discussed in Section \ref{sec:motivation}. 
% For example, the application in Figure~\ref{fig:collatz_sparkrdd}  analyzes the Collatz program discussed in Section \ref{sec:motivation}. In that section, a developer identified the \codefont{solve\_collatz} method as a point of interest. After changing a single line (line 1) in Figure \ref{fig:collatz_hybridrdd} to leverage \tool's \textit{HybridRDD} API, the developer can specify the \codefont{solved} variable as their target UDF in order to investigate the effects of the \codefont{solve\_collatz} function. 
Using this extension, \tool automatically decouples the \textit{map} transformation of \codefont{solved} from its predecessor (\codefont{grouped}) to produce a function of type \codefont{RDD[(Int, Iterable[Int])]} => \codefont{RDD[(Int, Int)]} which includes the \codefont{solve\_collatz} function. 

% During its execution, one particular task is responsible for a significant execution time to generate the \codefont{solved} dataset in line 9. To investigate this behavior, a developer interested in using \tool can provide \codefont{solved} as the target UDF for analysis.

% Given the resulting dataset definition, \tool determines the appropriate UDF by automatically investigating the program and extracting the preceding dataset transformation as function of the dataset’s parent input types.
% For \codefont{solved} in line 9 of Figure~\ref{fig:collatz_hybridrdd}, \tool identifies a function of type \codefont{RDD[(Int, Iterable[Int])]} => \codefont{RDD[(Int, Int)]} which represents the \codefont{map} operator that applies the \codefont{solve\_collatz} function.



%\gulzar{These are low-level details  about Spark. There should be a separate section called Implementation for this.} \jason{See latex comment for potential targets in each section that might be reorganized into Implementation section - not sure we have time to refactor though}
% UDF Isolation: the one paragraph on RDD setup that’s already marked
% Performance Monitors: could give more details on how the metrics are captured (SparkListener API),
% Mutations: could discuss the API/implementation (e.g. how data is collected in a partition-preserving fashion).
% Phased Fuzzing: Not sure what can be extracted here - perhaps the Prose section, though to be honest I’m also not particularly familiar with its implementation too.

%To isolate the user-defined UDF, we implement a wrapper, called {\it HybridRDD}, around Spark’s RDD API which tracks the transformations applied via an internal RDD, as shown in Figure~\ref{fig:collatz_hybridrdd}. It emulates Spark RDDs without implementing the RDD interface. A HybridRDD is a combination of {\it RDD transformation} (\eg \codefont{map} or \codefont{filter}) and {\it the input RDD with a specific type.} \tool derives the target UDF by analyzing the parent of a given \codefont{HybridRDD}.

%\jason{Moved Phase Fuzzing and Pseudo Inverse Inference via Program Synthesis sections to Section 4 as per reorg strategy}


\begin{table*}[th]
{    %\nocaptionrule
    \centering
        \scalebox{0.80}{\input{tables/metric_templates}}
		
    % \vspace{1ex}
    \caption{Monitor templates define how \tool detects specific symptoms and calculates feedback scores given a collection of values, denoted as $X$ in the predicates above and typically derived using the performance metrics in Table \ref{table:perf_metrics}.
    %In addition to the above parameters, each template can additionally specify a target stage position to restrict the scope of monitored partition performance metrics.
    }
    
    % \jason{Proposal: Examples for each may be redundant - how about a separate table with some examples (e.g., case studies) of translating english sentence to template + metric?}}
    % I think the focus should be on demonstrating how these are derived rather than how to mathematically compute some of these established functions.
    % see bookmark: https://docs.google.com/document/d/1TmAFAwpOzPSShQTZzPpap5rvInaIoJR_eN7IGp9cEQw/edit#bookmark=id.if6e9x7cekyh
    \label{table:metric_templates}
} 
% 		\vspace{-3ex}
%\vspace{-6ex}
\end{table*}
\begin{table}[th]
{    %\nocaptionrule
    \centering
        \scalebox{0.68}{\input{tables/perf_metrics}}
		
    \vspace{1ex}
    \caption{Performance metrics captured by \tool through Spark's Listener API to monitor performance symptoms, along with the associated performance skew they are used to measure. All metrics are reported separately for each partition and stage within an execution.}
    \label{table:perf_metrics}
} 
% 		\vspace{-3ex}
%\vspace{-6ex}
\end{table}
%\jason{Want to rewrite (rename section?) to indicate that we go Symptom -> Template + metrics.}

% \subsection{Performance Monitors as Fuzzing Guidance}\label{sec:perffeedback}
\subsection{Modeling performance symptoms}
\label{sec:perffeedback}
Existing test input generation techniques tend to optimize for metrics such as branch coverage. However, inputs with the same branch coverage can have distinct impacts on performance. Furthermore, such approaches do not account for performance symptoms and fail to monitor performance metrics such as task execution time, memory usage, and garbage collection time. In practice, performance skews can often be detected by patterns within such metrics. In order to guide test generation towards exposing specific performance symptoms, \tool provides a set of 8 customizable \textit{monitor templates} which model performance symptoms through 10 performance metrics derived through Spark's Listener API, shown in Tables \ref{table:metric_templates} and \ref{table:perf_metrics} respectively.
%For this purpose, we conclude \todo{X} kinds of metrics from \todo{Y} Stack Overflow posts related to performance skews, and design \todo{Z} performance metric template which can be customized by the user-defined symptom. 
Our insight behind these templates is that {\em DISC performance skews often follow patterns} and thus a user can specify the target performance symptom of test input generation by extending predefined patterns of performance metrics.


Each performance symptom is modeled by the combination of a \textit{monitor template} and a \textit{performance metric} (Figure \ref{fig:overview} label 2). A performance metric defines a distribution of data points associated with a UDF or program execution, which is then analyzed by monitor templates to detect whether the desired performance skew symptoms are exhibited. 
% Option for a 'simple' monitor example...\changed{For example, a monitor template could be used to check if any intermediate data partitions contain over 100 records}. 
In addition to detection, monitor templates also provide a feedback score which is used to guide fuzzing; newly generated inputs with higher feedback scores than previously observed are stored in an internal fuzzing input queue as candidates for future mutations. 


% \jason{I removed the previous bullet point examples as there were criticisms that they are too vague. Instead, I refer to the case studies for examples of the two skews we were able to reproduce. The previous text was repetitive (reiterating what causes each type of skew) and verbose (giving hypotheticals and an 'example' definition, which was not received well in the case studies).}

% \todo{Reference this to motivation instead.}Using the \textit{Collatz} example from Figure \ref{fig:collatz_hybridrdd}, a user could model a performance skew symptom by combining an \textit{IQROutlier(100.0)} template with the \textit{runtime} metric to detect the presence of any unusually slow partitions. 

As a simple example, consider a symptom where any partition's runtime during a program execution exceeds 100 seconds. This symptom can be defined by using the \textit{Runtime} metric and \textit{MaximumThreshold} monitor template, which then evaluates the predicate using the collected partition runtimes from Spark:
\begin{center}
$\max([Runtime]) \ge 100 s$.
\end{center}
Furthermore, the monitor template provides a feedback score corresponding to the largest metric (runtime) value observed. Additional examples of performance symptoms and their corresponding \tool definitions are discussed in the case studies of Section \ref{sec:evaluation}.
% START SKEW->DEFINITION BULLET POINTS
% Through the combination of monitor templates and performance metrics, \tool is able to capture a variety of performance skew categories:
% \begin{itemize}
%     \item \textbf{Data skew} arises from two reasons: (1) the key-based distribution of input data is non-uniform; or (2) the partition function is too weak to distribute data evenly across computation nodes. A few computation nodes are assigned with a significantly higher workload in both cases, causing a performance bottleneck. Given a symptom (\eg one task processes 20x more shuffle inputs than average), a developer could define a \textit{Leave One Out Ratio} template using the \textit{Shuffle Read Records} performance metric with a target factor of 20. 
%     \item \textbf{Computation skew} occurs when the content of a specific record triggers a compute-intensive program path inside a UDF. For example, a UDF that finds all permutations of an array is significantly slower on an array of size 10 than on an array of size 3. \\
%     %In other words, invoking the same UDF on a specific record or subset of records causes significant delay compared to other records. 
%         %Suppose a UDF finds all permutations of an array with a time complexity of \codefont{O(n!)}, where \codefont{n} is the array size. Invoking this UDF on a 10-length array would then be exceedingly slower than doing so on a 3-length array. \\
%       Given a symptom (\eg a single straggler task takes an abnormally high amount of time compared to others),  a developer could define an \textit{IQR Outlier} template which measures partition \textit{Runtime}.
%     \item  \textbf{Memory skew} occurs when the magnitude of constructed heap objects depends on the interaction between the UDF and its input. Suppose a UDF takes a node of a well-connected social-network graph as input and returns its edges as \codefont{Edge} objects. Processing a person with over 30 million connections will create immense memory pressure. \\
%      Given a symptom (\eg one task consistently fails with an out of memory error specifying \textit{GC Overhead exceeded}),  a developer could define an \textit{Error Detection} template which monitors for errors containing the substring "GC Overhead exceeded" and provide feedback using an underlying \textit{IQR Outlier} template that measures \textit{Garbage Collection}. 
% \end{itemize}

% END SKEW->DEFINITION BULLET POINTS

While \tool models many symptoms via the definitions in Tables \ref{table:metric_templates} and \ref{table:perf_metrics}, other symptoms may require additional patterns or metrics unique to a particular program. To support such symptoms, \tool also exposes endpoints for users to define their own monitor templates and performance metrics. In Section \ref{sec:evaluation}, we present one such example in which a custom metric is used to measure program-specific branch executions.
% jason: above is reworded to emphasize that this extension capability is a feature rather than a bug. We motivate it by admitting that \tool is limited in symptom scope but that we allow users to extend and thus capture additional symptoms.

% While \tool is oriented towards identifying performance symptoms, it is important to note that the monitor templates and metrics can be used interchangeably. In our evaluations in section \ref{sec:evaluation}, we demonstrate a use case which utilizes a custom control-flow-based metric rather than any of the performance metrics presented in Table \ref{table:perf_metrics}. Similarly, \tool provides the ability for users to define customized monitor templates for use with existing or custom metrics.
 
 
\subsection{Skew-Inspired Input Mutation Operations} \label{sec:mutation}
\begin{table*}[th]
{    %\nocaptionrule
    \centering
        \scalebox{0.68}{\input{tables/mutations}}
    \vspace{1ex}
    \caption{Skew-inspired mutation operations implemented by \tool for various data types and their typical skew categories. Some mutations depend on others (\eg due to nested data types);  in such cases, the most common target skews are listed.
    % in such cases, the listed target skew(s) are the most common usage, but actual skew may depend on underlying mutations. 
    % \changed{Changed: M\# identifiers used throughout paper, action-oriented names.}
    }
    \label{table:mutations}
} 
% 		\vspace{-3ex}
%\vspace{-6ex}
\end{table*}
A na\"ive way to mutate a data record would be either bit-level or byte-level mutation in which random bits (or bytes) are flipped in an input represented as a series of bits~\cite{afl}. Consider the Collatz program from Section \ref{sec:motivation}, which parses strings as space-separated integers.  When bit-level or byte-level mutations are applied to such inputs, they can hardly generate meaningful data that drives the program to a deep execution path since bit-flipping is likely to destroy the data format or data type. For example, modifying an input "10" to "1a"
% \fbox{\begin{minipage}[t][0.5em][t]{4em}\centering
% \centerline{\texttt{\footnotesize{(10,[1,0])}}} 
% \end{minipage}} to
% \fbox{\begin{minipage}[t][0.5em][t]{4em}\centering
% \centerline{\texttt{\footnotesize{(1a,[1,0])}}} 
% \end{minipage}} 
would produce a parsing error since an integer number is expected.
%in the first field. 
%Such meaningless inputs often fail due to issues irrelevant to performance, and are thus incapable of advancing fuzzing feedback metrics. 
Additionally, DISC applications include distributed performance bottlenecks such as data shuffling that are dependent on characteristics of the entire dataset and may be difficult or impossible to trigger with only record-level mutations. Designing mutations to detect performance skews in DISC applications requires that (1) mutations must ensure type-correctness, and (2) mutations should be able to manipulate input datasets in ways that comprehensively exercise the performance-sensitive aspects of distributed applications including but not limited to record-level operators and shuffling to redistribute data.
%\qian{I will restructure this para to emphasize naive mutations cannot take advantage of known types. parsing arguments of the target udf to get types + given types for original application's inputs.}

%Different from na\"ive mutations which ignore performance skew targets as well as input data types, 

\tool defines skew-inspired mutations to reduce the unfruitful fuzzing trials caused by ill-formatted data. The key insight behind this method is that the data types of isolated UDFs are inherently known through the \codefont{HybridRDD} implementation and can be used in conjunction with the target skew symptoms to tailor fuzzing mutations. For example, \tool targets data skew by defining mutations which alter the distribution of keys and values in tuple inputs as well as extend the length of collection-based fields.

Given the type signature of an isolated UDF, \tool returns the set of type-compatible mutations from Table \ref{table:mutations}. It then tailors the sampling probability to each mutation based on the skew category associated with the desired symptom (Figure \ref{fig:overview} label 3). Mutations aligned with the target skew category have increased probabilities while those that are not may see decreased probabilities. Table \ref{table:mutations} describes \tool's mutations along with their corresponding data types and target skew categories. Mutation probabilities are determined through heuristically assigned non-negative sampling weights, and mutations are selected through weighted random sampling.\footnote{https://en.wikipedia.org/wiki/Reservoir\_sampling\#Weighted\_random\_sampling}
% jason: could also make a mention that mutation weights are used over directly assigning probabilities as the mutations and probabilities will vary by data type and skew symptom. 
% The optimal mutations and weights may vary depending on the program and symptom to be reproduced. While the results in our evaluation demonstrate that mutation weights play a key role in \tool's ability to generate desired inputs, the challenge of identifying the optimal configurations remains an open problem for future work.

% \todo{Remove example/reference motivation if anything.}
%  Jason: removed for redundancy/lack of value. 
% As an example, consider the target UDF in Figure~\ref{fig:collatz_hybridrdd} with input records of type \codefont{(Int, Iterable[Int])} as well as an \textit{IQROutlier} monitor template which measures partition \textit{Runtime}. \tool identifies the 2-element tuple dataset mutations as well as \textit{RandomRecord} mutations corresponding to 2-element tuple, integer, and integer collections. 
% Because the \textit{Runtime} metric is typically associated with computation skew, \tool then decreases the probability of selecting mutations such as \textit{ValueEnumeration} which are not designed to target computation skew. \todo{Mutation references M\#}

% Not sure why there's a large gap here in latex...
% Goal: Explain that program input mutations are harder to weight and challenge of effectively mtuating program inputs. 
Although \tool also provides mutations for program inputs, their effectiveness is much more limited than that of mutations for intermediate inputs. Program inputs in DISC computing typically provide less information about data structure than UDFs (e.g., String inputs that must be parsed into columns) and, as noted in Section \ref{sec:udfisolation}, it is much more challenging to effectively mutate program inputs to explore performance skew deep in the execution path of a program.

% While these mutations are tailored for each UDF's type signature, it is also possible to generate mutations for program inputs. For example, the Collatz program's \codefont{String} input type combined with the previous \textit{Runtime}-based \textit{IQR Outlier} template can be used to identify the \textit{ReplaceSubstring} mutation for fuzzing. However, program inputs in DISC computing typically provide less information about data structure than UDFs (\eg String inputs that have not been parsed into columns) and, as noted in Section \ref{sec:udfisolation}, it is much more challenging to effectively mutate program inputs to explore performance skew deep in the execution path of a program.

\subsection{Phased Fuzzing} \label{sec:phasedfuzzing}
%\subsubsection{End-to-End Fuzzing with Improved Seeds}\label{sec:program_fuzzing_broken}
%\tool's ultimate goal is to generate test inputs to effectively trigger performance skews for a given application. To accomplish this, it requires as input an initial seed input for the application as well as the isolated UDF (Section \ref{sec:udfisolation}) and monitor template (Section \ref{sec:perffeedback}). 

\tool uses a \textit{phased fuzzing} approach to generate test inputs for the entire application. First, it uses the mutations from Section \ref{sec:mutation} to fuzz the specified UDF and produce a UDF input that triggers the target symptom.
%jason: simplifying - we can assume the mutations are provided...
%it uses the UDF schema and monitor template to identify an appropriate weighted set of mutations (Section \ref{sec:mutation}), which are then used to fuzz the specified UDF and identify a skew-inducing UDF input. 
Next, \tool converts this UDF input to an application input using an inverse function. Finally, the newly produced application input is used as an improved seed for fuzzing the entire program.


\noindent\textbf{Step 1. UDF Fuzzing.}
In order to more precisely reproduce performance skews, \tool first fuzzes the targeted UDF in isolation as illustrated in Figure \ref{fig:overview} label 4. It generates an initial UDF input seed by executing the subprogram leading up to the target UDF, and adds this seed to an internally maintained input queue. \tool then initiates a feedback-driven fuzzing loop using a given monitor template as feedback and skew-inspired mutations as input mutations operators to apply to a randomly selected input seed from the input queue. Two outcomes exist for each fuzzing loop iteration: (1) the monitor template detects that the desired symptom is triggered, so \tool saves the mutated input and terminates the fuzzing loop or (2) the monitor template does not detect skew but returns a feedback score that is better than previously observed, so \tool adds the mutated input to the queue, updates the best observed score, and resumes fuzzing with the updated input queue.

%Upon termination of the fuzzing loop, \tool has identified a UDF input which reproduces the target symptom. 
%Optionally, users may also specify an upperbound on the loop duration; if the duration is exceeded, \tool returns the stored input with the most desirable feedback score observed so far.
% Outdated but potentially useful doc for outline/reference, originally for SoCC: https://docs.google.com/document/d/1HutcplJY6LparkLzwm28UcAvDjZi1uM1eVLRkuwuFC0/edit?ouid=110746768153750189730&usp=docs_home&ths=true

% \tool fuzzes the target UDF by using the \textit{intermediate input mutations} to produce new inputs. These inputs are then executed by the UDF and the execution is monitored by the \textit{metric template}. If a newly mutated input appears to reproduce or come closer to reproducing the performance symptoms described in the \textit{metric template}, it is added to the collection of input seeds for mutation. At the same time, any generated inputs which reproduce the performance symptom defined by the \textit{metric template} are saved and used in \tool's subsequent step. \todo{this has overlap with the metric template definition/discussion in 3.4}. \todo{Do we need examples of input seed and corresponding intermediate seed? How much background knowledge is provided on seeds} \jason{regarding seeds: it's discussed in intro paragraph on "Fuzz testing has been proven..." - feel free to simplify where necessary.}


% Jason: Removed on 4/13 as we don't have enoguh Prose usage to justify.
% \begin{table}[t]
%     \centering 
%     \scalebox{0.85}{\input{tables/prose_results}}
    
%     \caption{Original input and intermediate output for the \textit{Collatz} program. Prose \cite{prosecode} gives an inverse function using \textbf{Intermediate Output} as input and \textbf{Original Input} as output.}
%     \label{table:prose_example}
%     %\vspace{-2ex}
% \end{table}


\noindent\textbf{Step 2. Inverse Function}
%Pseudo Inverse Inference.}
% Jason: changed because we aren't really selling the inference aspect/the techniques aren't available yet.

As \tool's objective is to produce program inputs which trigger performance skew, it needs some way to translate UDF inputs into program inputs. Intuitively, after generating the skew-inducing inputs for a target UDF, we can derive the original application's inputs by applying phased fuzzing to the portion of the program leading up to the UDF, with the goal of producing outputs which are equivalent to the UDF input we generated. However, this approach is not ideal in practice because it is difficult to guide fuzzing towards a specific output record (as opposed to a pattern or characteristic), resulting in many additional and potentially expensive Spark program executions.
%\jason{Other drawbacks include: requiring mutation definitions for these intermediate types (but see note below about recursive fuzzing), difficulty in reproducing outputs rather than behaviors/patterns.} 
To overcome these challenges, \tool requires users to define an \textit{inverse function} which directly converts intermediate UDF inputs to application inputs. 
% This definition can be determined in a variety of ways.
% data conversion techniques in program synthesis

As inverse functions cover the portion of a program preceding the target UDF, their logic does not require knowledge of the target UDF itself. Furthermore, they are not restricted by the target symptom that \tool aims to reproduce. As a result, inverse functions can be defined outside of \tool's \textit{phased fuzzing} process and are often simple enough for a developer to manually define in a matter of minutes. For example, Figure \ref{fig:collatz_inverse_fn} illustrates a simple inverse function for the \CollatzProgramName program discussed in Section \ref{sec:motivation}.
% For example, the \textit{Collatz} program's inverse function inverts the grouping and parsing logic defined in Figure \ref{fig:collatz_sparkrdd} (lines 3-7) and is shown in Figure \todo{Reference figure once labeled}. 

Automatically inferring inverse functions remains an open problem. While some dataflow operators may have clear inverse mappings, the logic of UDFs within those operators can vary greatly. Program synthesis offers some promise for automatically defining inverse functions. For example, Prose \cite{prosecode} supports automatic program generation based on input-output examples. However, such techniques are not currently designed to support DISC systems out of the box and require nontrivial extension in order to support key features such as distributed dataset inputs and shuffling.
%jason: not a big fan of above discussion. A future works section may be more appropriate.

% In the motivating example, we leverage Prose~\cite{prosecode}, a program synthesis tool, to generate a C\# version of an inverse function based on provided inputs and outputs. As shown in Table~\ref{table:prose_example}, Prose generates the inverse function for \texttt{Collatz}'s first three RDD transformations. Although this function may not be fully correct, it is still sufficient for \tool's requirement of producing input datasets. However, existing limitations require some additional developer intervention for adapting these inverse functions to \tool. First, language differences between Prose and \tool require a language conversion into a Scala/Java-based implementation. Second, some dataflow operators (\eg \codefont{groupByKey}) are not readily defined in Prose; in such cases, a developer must implement a corresponding 'inverse' operation (\eg \codefont{flatMap}). While this conversion process is manual in \tool's current implementation, we believe future work can help automate the language conversion and extend Prose to support dataflow operators.

% \changed{The challenge of identifying suitable inverse functions remains an open problem, as Prose and other automated program analysis techniques are not always sufficient or capable of analyzing DISC programs. One major obstacle is that such automated approaches would need to support a wide variety of input and output types; in our investigation, we found that Prose primarily supported String operations such as \textit{substring} but lacked support for other data types. However, \tool does not strictly require automatically generated inverse functions. In the event that such techniques are unusable or impractical, developers may also define their own inverse functions using domain knowledge about the program being investigated.}

\noindent\textbf{Step 3. End-to-End Fuzzing with Improved Seeds.} \label{sec:program_fuzzing}
A prior study~\cite{fuzzingevaluation} found substantial fuzzing performance variations based on the quality of seeds. Through the preceding steps, \tool is able to identify program inputs that are correlated with symptom-replicating UDF inputs. In the final step, our approach leverages these derived inputs as improved seeds for fuzzing the entire application as shown in Figure \ref{fig:overview} label 5. During this process, \tool reuses the same monitor template for detecting performance symptoms, but a different set of program input mutations corresponding to the program's input schema. This results in a fuzzing loop similar to the one used in fuzzing the intermediate UDF, but which generates symptom-producing program inputs rather than UDF inputs. 

% \changed{In cases where the inverse function accurately preserves the symptom-causing properties of an input dataset, this process typically terminates without requiring additional mutations. 


%\section{Implementation}

\begin{comment}
% jason: commented out this old block as it has been replaced since adding the mutations table.
For this UDF, \tool generates a variety of mutations which include but are not limited to: \todo{Update this to reflect the appropriate mutations from the mutations table, according to UDF input type.}
\begin{itemize}
    \item Random Key: Mutating a record's key to a new random value.
    \item Random Value: Mutating one or more items to new random values within a record's iterable value.
    \item Key Append: Appending record(s) with the same key but different iterable integer values.
    \item Value Append: Appending record(s) with the same value but different integer keys.
    \item (Iterable) Value Extension: Mutating an existing record by appending additional integers to its iterable value.
\end{itemize}
Given the \textit{partition runtime} \codefont{IQRTemplate} described in Section \ref{sec:perffeedback}, \tool also upweights the \textit{Value Extension} mutation as longer iterable values might increase runtime, and also downweights the \textit{Key Append} mutation as it is more typically associated with data skew rather than computation skew.

%\tool parses the argument of the isolated UDF (described in Section~\ref{sec:phasedfuzzing}), followed by producing a corresponding mutation for each data type. For the target UDF in Figure~\ref{fig:collatz_hybridrdd}, the \codefont{HybridRDD} in lines 9-10 shows that this UDF maps an input \codefont{RDD[(Int, Iterable[Int])]} to an output \codefont{RDD[(Int, Int)]}. When the first column of an input RDD is selected for mutations, \tool generates random integer numbers to reflect the \codefont{Int} type. 


\tool supports the mutation operators shown in Table \ref{table:mutations}. The mutations selected for fuzzing depend directly on the given UDF schema and performance symptoms. \todo{Perhaps a bit more discussion here}. 
\jason{This paragraph and list will be removed in favor of the table under construction}\tool is equipped with the following mutation operators:
\begin{itemize}
\vspace{-2pt}
\item{\bf Value Mutation (M1)} modifies a non-structure value according to its data type: \eg replacing an integer "4" with a new random integer "34".
\item{\bf Data Column Mutation (M2)} modifies the data value of a selected column in a tuple-based record based on its data type: \eg modifying the decimal value of \fbox{\begin{minipage}[t][0.5em][t]{4em}\centering
\centerline{\texttt{\footnotesize{bus,0.45}}} 
\end{minipage}} to \fbox{\begin{minipage}[t][0.5em][t]{4em}\centering
\centerline{\texttt{\footnotesize{bus,1.45}}} 
\end{minipage}}. This mutation typically depends on \textit{M1} for each of its columns.

%\item{\bf Crossover Mutation}

\item{\bf Key Replication Mutation (M3)} replicates data records mapped to the same key multiple times.

\item{\bf Key Append Mutation (M4)} appends data records with the same key but different values generating from an initial input record combined with \textbf{M1}. 
% jason: took this out because byte mutation is more of a base-level mutation.
% \item{\bf Byte Mutation (M3)} randomly flips one or several bytes.
\end{itemize}
\end{comment}


==> asplos_outdated/evaluations_asplos.tex <==
% 3/14/22 jteoh: This mostly reflects the ASPLOS '22 submission in Aug 2021, retained for reference.
\section{Evaluation}
\label{sec:evaluation}

\begin{comment}
\jason{Revising outline with the following high-level goals (until "END OUTLINE" comment)}:
RQ1: Fuzzing speed-up (total time until result, but also a secondary question of time per iteration while noting that 'good' iterations are going to be slower on average!)\\
RQ2: Fuzzing efficiency/accuracy (number of trials)\\
RQ3 (stretch): efficiency of reverse fn (compared to match fuzzing, which is nonideal as described in approach).

For evaluation results of total time, include a breakdown of time spent in each phase (UDF, reverse fn, and end-end fuzzing). 
Actual evaluations required: \\
(1) baseline: end-to-end fuzzing with fixed seed input (no queue size increase), schema-aware String mutations but no weights. \\
(2) PerfGen: phased fuzzing with UDF fuzzing, reverse fn, end-end fuzzing. Record time to first input, reverse fn time, time to program input, number of iterations in each phase.\\
(3 - stretch): Match fuzzing on program prefix trying to match UDF input from (2) - store/save/specify the seed file for efficiency if needed.

\jason{END OUTLINE}
\end{comment}

We evaluate \tool by posing the following research questions:
\begin{description}
% guidance metric
%\item[RQ1] {How much speed-up can \tool achieve by using performance monitors as a guidance metric as opposed to coverage-based guidance metric?} \jason{I thought we decided not to support this?}
% targeted fuzzing, phased fuzzing 
\item[RQ1] {How much speed-up can \tool achieve by phased fuzzing, as opposed to naive fuzzing?}
% in this case, we assume that the reverse function is unavailable and try again from the beginning by comparing the intermediate results against expected outputs in a phased manner.  % fuzz fn first, then rerun f0,f1, ..fn-1 all in sequence to check whether the intermediate output results are the same as fn's inputs
 \item[RQ2] {How much improvement in fuzzing accuracy does \tool provide through improved fuzzing seeds, as opposed to using the initial seed with naive fuzzing?}


RQ1 assess the overall time saving achieved by \tool's phased fuzzing approach that constructs intermediate inputs first, monitors performance symptoms in the target function, and uses the knowledge of intermediate inputs to guide input mutation steps. RQ2 measures the reduction in fuzzing iterations required to generate an input which triggers the desired performance skew symptoms when using the derived input seed from \tool's phased fuzzing approach. 
%\jason{This paragraph and Evaluation setup repeat a lot of the same information that is already present in the case study. Not sure if we should remove entirely or deduplicate somehow. (This also needs to be written under the assumption we have just the one case study now).}

%We investigate a case study described in Sections \todo{X}. These case studies come from \todo{Sources - I think Collatz is original? check with Qian + Jiyuan. Remainder come from BigDebug I think, though we've also made modifications to produce performance skews under certain conditions} \qian{Collatz is originally from~\cite{collatz}, we included it in Bigfuzz}, and their corresponding UDFs were identified from executions with datasets that were observed to produce performance skew. Monitor templates are determined according to the observed performance skew, and input seeds are derived from separate samples of existing input data that do not trigger any code errors or performance skew.

% Reach RQ
% \item[RQ3] {How much efficiency and effectiveness can be achieved through a reverse function synthesis?}
% in this case, we assume that a reverse function is synthesizable 
% We assess the trade-offs between the overall time saving, the time allocated for targeted fuzzing, and the time spent on synthesizing and running a reverse function.

% Optional additional RQ, but hard to evaluate without a 'base' set of mutations
% \item[RQ?] {How much speed up can \tool achieve by incorporating schema-aware input mutations?}
% in this case, we may need to justify where and how schema-aware input mutation operators come from. So it would be nice if such schema-aware input mutations can be learned from by comparing more than one seed inputs that trigger performance bugs. 

\end{description} 

\noindent{\bf Evaluation Setup}.
%\todo{Heavy overlap with Collatz case study - don't think we really need to explain setup. Possibly the overall comparison process but definitely not the arguments/parameters}.
%We evaluate \tool with each case study program, its corresponding input seed, the identified UDF, and a monitor template matching the expected performance skew. Inverse functions are assumed to have been derived ahead of time. UDF fuzzing is applied until an intermediate input is found, after which the UDF input is translated to an improved program input seed and end-to-end application fuzzing is executed until a skew-inducing program input is identified.  
For our baseline, we compare against a simplified version of \tool that does not apply phase fuzzing to produce intermediate inputs. Instead, this baseline version fuzzes the original program with the same monitor template but only the initial seed input. Similar to the \tool setup, this version fuzzes the program until a skew-inducing input is identified. For both versions, we use the same set of mutations for fuzzing the original program so that the only difference is the initial input seed. All evaluations are run using Spark 2.4.4's local execution mode on a single machine running macOS 10.15.7 with 16GB RAM and 2.6 GHz 6-core Intel Core i7 processor. 

\subsection{Case Study: Collatz Conjecture}
% Current Reference doc: https://docs.google.com/document/d/1JUIl0C94q4oUvENzKiqBaKNPyGmsD7vJ1yHolcOypDI/edit#
% Old one: https://docs.google.com/spreadsheets/d/1vxNp7JSOr-M-H0B0rh7kDQaCnrHH3uchQ5awwj8yGD0/edit#gid=724642834
The Collatz Conjecture program is adapted from \cite{collatz} and is shown in Figure \ref{fig:collatz_hybridrdd}. The program takes as input a string dataset consisting of space-separated integers. It splits each string into its individual integers, then applies the \codefont{solve\_collatz} function shown in Figure \ref{fig:solve_collatz} to compute a numerical value based on each integer's Collatz sequence length. 
\begin{figure}[t]
\centering 
\input{code/code_collatz_solve_equation_udf}
\vspace{-2ex}
\caption{The \codefont{solve\_collatz} function used in Figure \ref{fig:collatz_hybridrdd} to determine each integer's Collatz sequence length and compute a polynomial-time sum based on the sequence length.}
\label{fig:solve_collatz}
\end{figure}

We previously observed that this program exhibited symptoms of computation skew in at least one execution. In particular, we noticed that one partition in the first stage takes dozens of times longer to compute than the others with no noticeable difference in record count or memory usage. However, tracing such a symptom back to a skew-inducing input is highly challenging. As a result, we choose to use \tool to generate test inputs which reproduce this performance skew.

As our first step, we encode the desired performance symptoms into a monitor template. Given that the observed behavior affected runtime but not memory or data distribution, we choose to analyze the \textit{Runtime} metric via an \textit{IQR Outlier} monitor template with a specified distance threshold of 100. 

Next, we identify a UDF for targeted fuzzing. Given the complexity of the \codefont{solve\_collatz} function, we decide to isolate the corresponding \codefont{solved} transformation. As a result, we isolate a UDF that consumes \codefont{(Int, Iterable[Int])} and produces \codefont{(Int, Int)} outputs.

Based on the monitor template and the UDF type signature, \tool identifies the following mutations from Table \ref{table:mutations} and weights them as follows\footnote{Mutations in parentheses are combined to match the required UDF input type.}: 
\begin{itemize}
    \item RandomInteger\\(RandomRecord+TupleElementMutation), 1.0
    \item CollectionConcatenation\\(RandomRecord+TupleElementMutation), 1.0
    \item CollectionElementMutation\\(RandomRecord+TupleElementMutation), 5.0
    \item KeyEnumeration, 0.5
    \item ValueEnumeration, 0.5
    \item DuplicateKeyGeneration, 0.5
    \item DuplicateValueGeneration, 0.5
\end{itemize}
 Due to the monitor template's focus on partition runtime skew, \tool decreases the weights of the data skew mutations. At the same time, it increases the weight of \textit{CollectionElementMutation} to encourage fuzzing to explore each item within the \codefont{Iterable[Int]} value.

Finally, fuzzing requires a program input seed as a basis for mutations. For simplicity, we create a simple program input seed with the following partitions, with horizontal lines indicating partition divisions. :
\begin{center}
\begin{tabular}{r}
Program Input\\
\hline
"1" \\
\hline
"2"\\
\hline
"3"\\
\hline
"4"\\
\hline
\end{tabular}
\end{center}
%\jason{Could include output snippet as well, but it's not actually relevant to the example}
When testing this seed input, \tool finds that no performance skew is exhibited. Furthermore, manual inspection of each element indicates that all integers have relatively short Collatz conjecture sequence lengths, with the longest being a sequence of length 7 for the integer "3".

\tool's phased fuzzing approach fuzzes the isolated UDF. It starts by first partially running the program with the provided program input seed to determine an appropriate UDF input seed.
\begin{center}
\begin{tabular}{r}
UDF Input\\
\hline
(4, [1]) \\
\hline
(1, [1])\\
\hline
(2, [1])\\
\hline
(3, [1])\\
\hline
\end{tabular}
\end{center}
Using this UDF input seed and the mutations noted earlier, \tool fuzzes the UDF. After 34 iterations and 30385 ms, it produces a skew-inducing UDF input by applying the \textit{RandomInt} mutation (in combination with \textit{TupleElementMutation} on the tuple key) to alter the bolded record key from "1" to "1497909577":
\begin{center}
\begin{tabular}{r}
UDF Input\\
\hline
(4, [1]) \\
\hline
(\textbf{1497909577}, [1])\\
\hline
(2, [1])\\
\hline
(3, [1])\\
\hline
\end{tabular}
\end{center}
"1497909577" has a much longer Collatz conjecture sequence length of 183 numbers which, when combined with the \codefont{solve\_collatz} function, results in significantly longer computation time compared to the remaining records. As a result, \tool has successfully identified a UDF input that produces the desired performance skew.

As \tool aims to trigger performance skew with program inputs, it converts this UDF input into a program input through the use of an inverse function. Through a combination of Apache Spark operator analysis and program synthesis via Prose \cite{prosecode}, we define the following inverse function to convert a UDF input  to a program input:
\input{code/code_collatz_inverse_fn}
% \jason{There's some drawbacks to this inverse function, e.g. it's impossible to reverse a flatMap if there's no common key to regroup records by. I'm not sure it's worth mentioning here though.}
Due to existing limitations which require manual intervention to adopt the Prose function into \tool, the process of generating this inverse function takes up to 5 minutes that includes the initialization time for Prose, feeding inputs, and C\# to Scala conversion. 

\tool then applies this inverse function on the UDF input generated from fuzzing, which produces the following program inputs after 137 ms:
\begin{center}
\begin{tabular}{r}
Program Input\\
\hline
\hline
"4"\\
\hline
"1497909577"\\
\hline
"1"\\
\hline
"3"\\
\hline
\end{tabular}
\end{center}

Finally, \tool uses this input along with \textit{ReplaceSubstring} mutation to fuzz the program inputs for the same performance symptom defined by our existing monitor template. In this case, only one iteration is required  as \tool verifies tests the inverted input, which takes 27180 ms, and finds that it is already sufficient for triggering the desired performance skew symptoms. 
%\jason{See note in approach, we might want to discuss how it's sometimes sufficient to simply convert UDF input -> program input with the inverse function. Alternatively consider an additional extension/evaluation to produce more inputs, e.g. reuse UDF-based seed and run for X minutes to identify new inputs to compare speed against the baseline.}

As a baseline, we also use \tool to directly fuzz the program inputs using our initial seed input as opposed to the improved seed identified through UDF fuzzing and the inverse function. After 58426 iterations and 2668253 ms (almost 45 minutes), the following result is produced:
\begin{center}
\begin{tabular}{r}
Program Input\\
\hline
"1"\\
\hline
"2"\\
\hline
"3"\\
\hline
% A909
"\includegraphics[width=2mm]{images/9.pdf}4"\\
\KLNine
\hline
\end{tabular}
\end{center}
% \todo{Jason: I need help fix a special character which does not show up before the "4" - it should be kayah li 9 (unicode U+A909). Google suggests using \\usepackage[utf8x]\{inputenc\} as well as trying a different unicode-compatible compiler (I tested XeLaTeX with no luck)}
% update: Qian found a workaround with using \includegraphics, go Qian!

While the final record does not immediately appear to be numeric, manual investigation revealed that the first character actually corresponds to "9" in the Kayah Li alphabet\footnote{https://en.wikipedia.org/wiki/Kayah\_Li\_alphabet} and is considered a valid integer string in Scala.

% Results spreadsheet for Collatz https://docs.google.com/spreadsheets/d/1oK1u_iZckc9R10DlPgW_JNW_2OYJu0L6gFO8jxFmiW4/edit?usp=sharing
%metrics: Speedup of phased vs naive fuzzing. Speedup of improved input seed [evaluation only, less significant]. Improvement in fuzzing accuracy. 
\begin{table}[t]
{    %\nocaptionrule
    \centering
    % original scale 0.68
        \scalebox{0.8}{\input{tables/collatz_results}}
        
		
    \vspace{1ex}
    \caption{Fuzzing times and number of iterations for the Collatz case study. \textit {Phased Fuzzing} represents the entire \tool approach and includes \textit{UDF Fuzzing}, time spent applying the inverse function to the result of \textit{UDF Fuzzing}, and \textit{Program Fuzzing with Improved Seed}.}
    \label{table:collatz_results}
} 
		\vspace{-3ex}
%\vspace{-6ex}
\end{table}

The results for both \tool and baseline are summarized in Table \ref{table:collatz_results}. Comparing this baseline approach to \tool's phased fuzzing, using \tool leads to a 46X speedup in workload generation speed if the inverse function is predefined. Including an upperbound of 5 minutes overhead for identifying an inverse function, \tool achieves almost 7.5X speedup compared to the baseline. When fuzzing the original program, using an improved input seed derived from UDF fuzzing results in 98X speedup compared to fuzzing with the original input seed. Furthermore, the improved input seed produces 58425X improvement in fuzzing accuracy compared to the original input seed. In other words, baseline setup produces over 58425 inputs before reaching the required performance symptom whereas \tool does the same in 1 iteration. Finally, \tool uses skew-inspired mutations to fuzz the isolated UDF with 1717X better accuracy compared to fuzzing the full program, thus highlighting the challenge of fuzzing paths deep inside programs and the potential for more accurate fuzzing mutations through program slicing. 
%\jason{Could potentially use more interpretation/significance discussion here if time permits}.
% generates an input workload 46X faster than is able to reproduce the desired performance skew in \todo{X}\% of the time required for the baseline fuzzing approach, despite spending \todo{Y}\% of its time identifying an improved input seed. Additionally, we find that the improved input speed results in only \todo{Z}\% of the total number of fuzzing iterations required by the baseline fuzzing approach. The results are illustrated in Figure \todo{Insert figure for time breakdown, summary for number of iterations. This section is just math from the existing results}.

% \jason{Proposed results 'higlights' to be later copied abstract, intro, extended abstract} We evaluate \tool using an in-depth case study which demonstrates that \tool achieves 46X speedup compared to traditional fuzzing approaches when generating workloads which exhibit specified performance skew symptoms. Additionally, the improved input seed identified in \tool's phase fuzzing approach improves the fuzzing success rate of the original program by 58425X.


\begin{comment}
\jason{Looking at time remaining, doesn't seem likely that I'll get to a second case study.} 
\subsection{Case Study B: GENERIC TEMPLATE}

\noindent{\bf Program description} TODO: Program (description + code), origins, example input + output, observed skew (location + symptom), initial input seed

\noindent{\bf Isolated UDF} Which UDF is chosen, its schema, and the UDF input seed. [note: next few sections can be potentially merged into one]

\noindent{\bf Monitor Template} How the skew is translated to a template. 

\noindent{\bf Mutations} Which mutations and weights, derived from UDF + Monitor Template. 

\noindent{\bf Inverse Function} Portion of program that it corresponds to, what the rev function looks like when converted.

\noindent{\bf Phased Fuzzing} Paragraph 1: The UDF Fuzzing results - example snippet of output, time taken, number of iterations.

Paragraph 2: Result of applying the inverse function to produce a program input.


Paragraph 3: Using result as seed input for end-to-end fuzzing - example snippet of output, time taken, number of iterations. Any other useful breakdown numbers too.

Paragraph 4: Baseline comparison: snippet of output if applicable, time taken, number of iterations.
\end{comment}

==> asplos_outdated/motivating_old_asplos.tex <==
% \todo{do we need a background section on fuzz testing and performance skew?}

\begin{figure*}[t]
    \centering
    \scalebox{0.95}{\includegraphics[width=\textwidth]{images/overview.pdf}}
    \caption{\bf \tool contains three novel components: phased fuzzing with inverse mapping, symptom-specific performance monitoring, and skew-inspired input mutations. \todo{Ref this in introduction or move to approach}}
    \label{fig:overview}
\end{figure*}


\section{Motivating Example} 
\label{sec:motivation}

% \gulzar{This sections contains a mixture of content from PerfDebug and the collatz case study. }
% \jason{Some gaps in logic and motivation here, but moving on for the sake of time}

To demonstrate the challenges of performance debugging and how \tool addressed such challenges, we present a motivating example adopted from prior work on performance debugging~\cite{teoh:socc:perfdebug}.


In this example, a developer uses a Spark program to calculate the frequency of movie ratings in a 21GB dataset of movies and their user ratings. A row in this dataset consists of a movie ID prefix followed by comma-separated pairs of a user ID and a numerical rating (1 to 5). A small snippet of this dataset is as follows:
\vbox{
\centering
 \vspace{1ex}
\noindent{\tt\small 
% m1:u1\_3,u324\_5,u514\_4,u866\_4,u912\_4,u978\_5 \\
% m2:u23\_1,u316\_2,u412\_2,u779\_1 \\
% m3:u108\_5,u150\_3,u237\_3,u405\_2, u941\_5 \\
% ... \\
% m486:u1\_5,u2\_5,u3\_5,u4\_5,...,u998\_5,u999\_5 
127142:2628763\_4,2206105\_4,802003\_3,...\\
127143:1027819\_3,872323\_3,1323848\_4,...\\
127144:1789551\_3,1764022\_5,1215225\_5,...\\
}
}
The developer writes a Spark application that uses a  \texttt{map} operator to extract the substring containing ratings from each row. Then it uses another \texttt{map} operator to find the distribution of ratings only for a single movie. In the next phase, it uses a \texttt{reduce} operation to aggregate rating frequencies from each row to compute the distribution of ratings across the entire dataset.


Once the job is launched, the developer notices the first stage of the job is responsible for over 98\% of the total program execution time. Upon further investigation into Spark performance metrics, the developer finds that a single task in this stage, Task 33, runs for 1.2 minutes while the remaining tasks finish much earlier; the median task time is 11 seconds, but Task 33 takes over 50\% longer than the next slowest task which completes in 51 seconds. Furthermore, the input data per partition is roughly consistent at 128MB. Other tasks which execute on the same machine perform normally, which eliminates the existence of a straggler due to hardware failures. Since the program contains identical code logic for each partition and the developer has confirmed roughly equal distributions of data, they suspect this behavior is an instance of computation skew.
%This is a pure computation skew symptom since the developer has confirmed the code logic is the same for all partitions and the data records are equally distributed.

The developer decides to investigate the cause of this delay. They start by investigating inputs corresponding to the slow task. However, they quickly find that doing so is infeasible as the 128MB input consists of millions of records, too many to easily inspect manually. Thus, it is difficult to understand what characteristics of the data may have triggered the observed performance issues.

% \jason{This feels incomplete/could better emphasize how finding the cause or reproducing the input is difficult} To investigate which dataset characteristics caused the program to show disproportionate delays, the developer requests to see a subset of original input records accountable for the slow task. This manual inspection is infeasible since it contains 128MB of raw data and comprises millions of records. 

To avoid encountering such problems with large-scale production data, the developer may use better performance testing tools to reproduce the skew. Suppose the developer uses an AFL-like na\"ive fuzzing technique in an attempt to find such skew-inducing inputs. It treats the entire input dataset as bit series and randomly flips several bits or bytes. This process inevitably involves many trials because performance skews are rare events, and the na\"ive probability of hitting the skew-inducing partitions in the same data size is marginal as each partition can contain millions of data records. Additionally, AFL-like fuzzing uses code branch coverage as guidance to drive test generation to rare execution paths, which cannot account for the execution time of different input records with identical coverage. 

The developer decides to use \tool to expose performance skews before running the application at full scale. As a first step, \tool requires the user to encode the desired performance symptoms into one of the monitor templates defined in Table \ref{table:metric_templates}. Given that the observed behavior affects the task runtimes, the developer choose to analyze the \textit{Runtime} metric via an \textit{IQROutlier} monitor template. Next, the developer identifies a UDF for targeted fuzzing, following a decreasing order of complexity within the affected stage. Thus, the UDF in the second map operator is selected first. 

Based on this monitor template and the UDF type signature \codefont{(String, Iterable[Int])}, \tool determines the appropriate skew-inspired mutations from Table \ref{table:mutations} which include mutations such as \textit{ReplaceSubstring}, \textit{CollectionConcatenation}, and \textit{KeyEnumeration}. Since the monitor template focuses on computation skew via runtime, \tool increases the \changed{probability} of applying mutations tailored towards computation skew (\eg \textit{CollectionConcatenation}) and decreases the probability of those which solely target data or memory skew (\eg \textit{KeyEnumeration}).\todo{Replace with M# identifiers in table}. \todo{Forward reference, but state which mutations and mention that some are upweighted?}
 %Due to the monitor template's focus on partition runtime skew, \tool increases the weight of \textit{CollectionElementMutation} to encourage fuzzing to explore each item within the \codefont{Iterable[Int]} value.

\tool's phased fuzzing approach fuzzes the isolated UDF. It starts by partially running the program with the provided input seed to determine an appropriate UDF input seed. Using this UDF input seed and the earlier identified mutations, \tool fuzzes the UDF to produce an input which triggers computation skew. After a few iterations, it produces a skew-inducing UDF input by applying the \todo{UPDATE+ReplaceIdentifier}\textit{CollectionConcatenation} mutation to greatly increase one record's movies ratings list length by duplicating the values. This resulting UDF input thus contains the original UDF inputs, but with one record possessing a substantially longer value (ratings) list than the remaining record. \tool then converts this UDF input into a program input through the use of a \changed{user-provided} inverse function, which joins these ratings together to produce a final dataset of program input strings which reproduce the desired performance skew. % final skew-inducing program input strings. 
%At this point, the developer is not only able to reproduce the computation skew previously observed, but can easily investigate how mutations were used to alter an input dataset to trigger this skew.

%the developer may use this input to trigger hidden application performance limitations that surface only at a large scale. 

\todo{Update approach diagram, add references to examples.}


\begin{comment}


%e.g. starting from SO post with symptoms, but no provided data → how do we replicate? (perf replication)benchmarking workload generation: Input symptom(s) -> produce a representative workload}

%\todo{SO post no.39699728}
%Discussed with Jason. We think this post is promising as a motivation example. in particular: "the problem I am facing is out of 70 partitions 68 partitions gave result in around 20\% of time compared to the time taken by last 2 partitions. I have checked my data is equally distributed on all partitions , and even checked with different sample data also." also more motivation from one of the responses: "NLP tasks can take variable amounts of time depending on the data factors. For example, Stanford's CoreNLP takes a very long time to do NER on long sentences (time goes up with the square of the number of tokens in the sentence)."

\miryung{page allocation: 0.75 page? I suggest to structure this section as follows.} 

\miryung{(paragraph A-5 sentences). start with SO post that maps to memory skew symptom or computation sk[ew symptom, state that it is difficult to reproduce a performance error due to not having.}\qian{why not use fig3 as a motivating example??Drafting paraC D E is difficult because there is no code example in SO post.}
This section discusses one real-world example based on Stack Overflow post No.~39699728~\cite{39699728} to show the benefit of \tool. In this post, the developer uses a Spark program with \codefont{map} and \codefont{flatmap} functions to do sentimental analysis of comments. This program runs successfully on Spark; however, the developer notices a sign of poor performance that {\it ``68 out of 70 partitions gave result in around 20\% of time compared to the time taken by last 2 partitions.''} This is a pure computation skew symptom since the developer has confirmed the code logic are the same for all partitions and the data is equally distributed. One of the responses points out that NLP tasks can take variable amounts of time depending on the data factors. For example, Stanford's CoreNLP~\cite{} takes a very long time to do named-entity recognition on long sentences (time goes up with the square of the number of tokens in the sentence). Though the developer briefly described the task of his/her program, reproducing this performance symptom is difficult due to lacking of corresponding inputs.

%\miryung{(parag B - 5 sentences, describe what it would take to generate the input using naive fuzzing} 
Suppose we use an AFL-like na\"ive fuzzing technique in an attempt to find such skew-inducing inputs. It treats the entire input dataset as bit series and randomly flips several bits or bytes. This process inevitably involves a considerable amount of trials because performance skews are rare event and the na\"ive probability of hitting the skew-inducing partitions in the same data size is approximately 2.86\% (= 2/70). In fact, this probability will be even lower since each partition can contain millions of data records. Additionally, AFL-like fuzzing uses code branch coverage as guidance to drive test generation to rare execution paths, which cannot account for the execution time of different input records with identical coverage.

\miryung{(parag C-5 sentences: a user extends to create a custom monitor. give an example of performance skew template, a user specifies the involved constants.}
\todo{need to understand more about performance templates. i.e., symptom->symptom-specific feedback metric monitoring, and how to customize.}

with perfgen, this develop can set the fuzzing objective as time(a)>threshold*average -> computation skew template -> customized perf metrics for this symptom. -> fuzz the program to max such perf metrics.

\miryung{parag D-5 sentences, describe how long it takes to find the input,  - describe the symptom of reproduced performance skew, read out  a few samples of inputs, explain why the performance symptom is caused by relating to the data,} 
\qian{This para D seems infeasible as no code available in the post => cannot read out a few detailed data samples.}

\miryung{parag E: summarize speed up and success rate comparison between naive fuzzing vs. \tool }





\end{comment}

==> case_studies/case_study_collatz_standalone.tex <==
% \newcommand{\CollatzProgramName}{\textit{Collatz}\xspace}
% \newcommand{\solvedRDD}{\textit{solved}\xspace}
% \soulregister{\CollatzProgramName}{7}
% \soulregister{\solvedRDD}{7}

\subsection{Case Study: Collatz Conjecture}
% \changed{\jason{Changed results discussion (at end) and added subsubsection markers (for sake of reference - in practice I think they may be clutter/unnecessary).}}
\jason{Planning to revisit this after updating the motivation, then backreferencing whatever is duplicated/unnecessary. The expectation is that this section will be much shorter after.}
% 4/18 - decided to rewrite anyways. With assumption that example inputs shown in approach figure.
\subsubsection{Setup.}
Suppose a developer is interested in the \CollatzProgramName program, adapted from \cite{collatz} and shown in Figure \ref{fig:collatz_hybridrdd}. Consuming a string dataset space-separated integers, the program splits each string into its individual integers and applies the polynomial-time \codefont{solve\_collatz} function shown in Figure \ref{fig:solve_collatz} to compute a numerical value based on each integer's Collatz sequence length. 

\begin{figure}[t]
\centering 
\input{code/code_collatz_solve_equation_udf}
\vspace{-2ex}
\caption{The \codefont{solve\_collatz} function used in Figure \ref{fig:collatz_hybridrdd} to determine each integer's Collatz sequence length and compute a polynomial-time sum based on the sequence length.}
\label{fig:solve_collatz}
\end{figure}

For simplicity, the developer starts with the minimal seed input shown in Figure \ref{fig:overview}, with each record separated into its own partition.
% When testing this seed input, \perfgen finds that no performance skew is exhibited. Furthermore, manual inspection of each element indicates that all integers have relatively short Collatz conjecture sequence lengths, with the longest being a sequence of length 7 for the integer "3".


\paragraph{Symptom.}
% IQR, 100x
The developer is interested in inputs that will exhibit severe computation skew in which one outlier partition takes significantly longer to compute than others during the \codefont{solve\_collatz} function in Figure \ref{fig:solve_collatz}, associated with the \solvedRDD variable (Figure \ref{fig:collatz_sparkrdd}, line 9). Choosing to use \perfgen to produce such an input, they combine the \textit{Runtime} metric with an \textit{IQROutlier} monitor template, specifying a target threshold of 100.0 so that severe computation skew will be reproduced.

% We previously observed that this program exhibited symptoms of computation skew in at least one execution. In particular, we noticed that one partition in the first stage takes dozens of times longer to compute than the others with no noticeable difference in record count or memory usage. However, tracing such a symptom back to a skew-inducing input is highly challenging. \gulzar{This will need more detail. The issues is that goal of fuzzing is to expose a perf symptom, which we have seen already with the previous execution. Now what is the benefit of reproducing the same symptom. It becomes a debugging problem if our goal is to find a precise input responsible.} As a result, we choose to use \perfgen to generate test inputs which reproduce this performance skew.

\paragraph{Mutations.}
The \solvedRDD RDD consumes \textit{(Int, Iterable[Int])} inputs. For this input type and the given computation skew symptom, \perfgen defines the following mutations and weights:
\footnote{Mutations in parentheses are combined to match the required UDF input type.}

\begin{itemize}
    % \item RandomInteger\\(RandomRecord+TupleElementMutation), 1.0
    % \item CollectionConcatenation\\(RandomRecord+TupleElementMutation), 1.0
    % \item CollectionElementMutation\\(RandomRecord+TupleElementMutation), 5.0
    % \item KeyEnumeration, 0.5
    % \item ValueEnumeration, 0.5
    % % \item DuplicateKeyGeneration, 0.5
    % %  While originally intended, this was not supported due to type and implementation limitations.
    % % (It's hard to generate a random iterable of values and would require more composition than currently supported)
    % \item DuplicateValueGeneration, 1.0
    
    % Referenced against mutations table.
    \item M1 (M10 + M7), 1.0
    \item M5 (M10 + M7 + M1), 5.0 % fixed bug: Needs to have a reference to the value-level mutation too.
    \item M6 (M10 + M7), 1.0
    \item M11, 0.5
    \item M12, 0.5
    \item M14, 1.0
    
\end{itemize}
%  Due to the monitor template's focus on partition runtime skew, \perfgen decreases the weights of the data skew mutations. At the same time, it increases the weight of \textit{M6} to encourage fuzzing to explore each item within the \codefont{Iterable[Int]} value.

% JASON RESUME HERE

\paragraph{Inverse Function.}
In order to invert lines 3-7 of the \CollatzProgramName program in Figure \ref{fig:collatz_sparkrdd}, the developer defines a function to flatten each group and extract each integer key as a string input:
\todo{Move this to approach as an example.}
\begin{figure}[t]
\centering 
\input{code/code_collatz_inverse_fn}
\vspace{-2ex}
\caption{The \CollatzProgramName inverse function to converts UDF inputs into inputs for the entire program.}
\label{fig:collatz_inverse_fn}
\end{figure}


\subsubsection{\perfgen Execution.}
\paragraph{UDF Fuzzing.}
\perfgen first executes \CollatzProgramName with the input data until reaching the target UDF, producing the UDF input shown in Figure \ref{fig:overview}. It then fuzzes the UDF using the earlier defined mutations and, after 3 iterations and 41,221 ms, produces the symptom-triggering UDF input (Figure \ref{fig:overview}, starred) by applying the \textiti{M14} mutation to add the bolded record.\footnote{
"474680340"'s Collatz sequence length is 192, while the remaining records' lengths are no more than 7.}

\paragraph{Program Fuzzing.}
\perfgen uses the inverse function to convert the symptom-triggering UDF input to the program input shown in Figure \ref{fig:overview}. It then tests this program to find that the symptom is still produced for this new input to the entire program, and no additional fuzzing is necessary.

\subsubsection{Baseline.}
We evaluate the \CollatzProgramName program under our baseline configurations and find that it produces a symptom-triggering input after 12,166 iterations and 937,071 ms:\footnote{Scala's integer parsing includes support for non-Arabic numerals.}
% Jason: I'm planning to remove most snippets, but Collatz is the only one still illustrated so it is retained here.
\begin{center}
\begin{tabular}{r}
Program Input\\
\hline
"1"\\
\hline
"2"\\
\hline
"3"\\
\hline
% A909
% "\includegraphics[width=2mm]{images/9.pdf}4"\\
% \KLNine
% \hline
"3\includegraphics[width=3mm]{images/38-2.png}"\\ 
\hline
\end{tabular}
\end{center}
% Credit goes to Qian for finding a workaroudn to include the unicode character - it should be kayah li 9 (unicode U+A909). Jason was otherwise unable to get the Google suggestion of \\usepackage[utf8x]\{inputenc\} as well as trying a different unicode-compatible compiler (I tested XeLaTeX with no luck)}. Thank you Qian!
% Update 4/11: Changing results, we now have Limbu Digit 3 and N'Ko digit 8
% ᥉߈
% "3\includegraphics[width=3mm]{images/38-2.png}"\\ 
% https://en.wikipedia.org/wiki/Limbu_script
% https://en.wikipedia.org/wiki/N'Ko\_script



\subsubsection{Discussion.}
%  11.17, 0.008%, 0.02%

\CollatzProgramName evaluation results are summarized in Table \ref{table:case_study_results}, with the progress of the best observed \textit{IQROutlier} feedback scores plotted in Figure \ref{fig:time_series}. 
% iterations, speed, and metric score discussion
Compared to the baseline, \perfgen's approach produces a 11.17X speedup and requires 0.008\% of the program fuzzing iterations. Additionally, \perfgen spends 49.14\% of its total input generation time on the UDF fuzzing process.
% Not planning to dive into it, but if necessary: This is because the actual input execution time dominated the program executions!
% Furthermore, the number of UDF fuzzing iterations required totals 0.02\% of the program fuzzing iterations required by the baseline.

While both configurations are able to successfully generate inputs which trigger the desired symptom, \perfgen is able to do so much more efficiently because its type knowledge allows it to focus on generating integer inputs while the baseline is restricted to string-based mutations which may fail the integer parsing process.

% \changed{Furthermore, the use of the improved input seed requires far fewer iterations compared to the original input seed. \perfgen is able to produce a symptom-triggering input in a single iteration, 1/58426 the number of iterations required by the baseline approach. This is possible because \perfgen directly targets the isolated UDF and is able to generate an intermediate input which successfully triggers the target symptom in 34 iterations, less than 0.06\% the number of iterations required for the baseline to produce inputs for the full program. This contrast demonstrates the challenges of fuzzing paths deep inside programs and the potential for more accurate fuzzing mutations through program slicing. In particular, \perfgen's type-aware approach is able to address the \textit{Collatz} program's expectation of numerical inputs while the baseline is restricted to string-based mutations.}

% Original ASPLOS: The results for both \perfgen and baseline are summarized in Table \ref{table:collatz_results}. Comparing this baseline approach to \perfgen's phased fuzzing, using \perfgen leads to a 46X speedup in workload generation speed if the inverse function is predefined. Including an upperbound of 5 minutes overhead for identifying an inverse function, \perfgen achieves almost 7.5X speedup compared to the baseline. When fuzzing the original program, using an improved input seed derived from UDF fuzzing results in 98X speedup compared to fuzzing with the original input seed. Furthermore, the improved input seed produces 58425X improvement in fuzzing accuracy compared to the original input seed. In other words, baseline setup produces over 58425 inputs before reaching the required performance symptom whereas \perfgen does the same in 1 iteration. Finally, \perfgen uses skew-inspired mutations to fuzz the isolated UDF with 1717X better accuracy compared to fuzzing the full program, thus highlighting the challenge of fuzzing paths deep inside programs and the potential for more accurate fuzzing mutations through program slicing. 
%\jason{Could potentially use more interpretation/significance discussion here if time permits}.

==> case_studies/old/case_study_collatz_old.tex <==
\subsection{Case Study: Collatz Conjecture}
\changed{\jason{Changed results discussion (at end) and added subsubsection markers (for sake of reference - in practice I think they may be clutter/unnecessary).}}

\subsubsection{Program Definition.}
The Collatz Conjecture program is adapted from \cite{collatz} and is shown in Figure \ref{fig:collatz_hybridrdd}. The program takes as input a string dataset consisting of space-separated integers. It splits each string into its individual integers, then applies the \codefont{solve\_collatz} function shown in Figure \ref{fig:solve_collatz} to compute a numerical value based on each integer's Collatz sequence length. 
\begin{figure}[t]
\centering 
\input{code/code_collatz_solve_equation_udf}
\vspace{-2ex}
\caption{The \codefont{solve\_collatz} function used in Figure \ref{fig:collatz_hybridrdd} to determine each integer's Collatz sequence length and compute a polynomial-time sum based on the sequence length.}
\label{fig:solve_collatz}
\end{figure}

\subsubsection{Symptom.}
We previously observed that this program exhibited symptoms of computation skew in at least one execution. In particular, we noticed that one partition in the first stage takes dozens of times longer to compute than the others with no noticeable difference in record count or memory usage. However, tracing such a symptom back to a skew-inducing input is highly challenging. \gulzar{This will need more detail. The issues is that goal of fuzzing is to expose a perf symptom, which we have seen already with the previous execution. Now what is the benefit of reproducing the same symptom. It becomes a debugging problem if our goal is to find a precise input responsible.} As a result, we choose to use \tool to generate test inputs which reproduce this performance skew.

\subsubsection{Monitor Template Definition.}
As our first step, we encode the desired performance symptoms into a monitor template. Given that the observed behavior affected runtime but not memory or data distribution, we choose to analyze the \textit{Runtime} metric via an \textit{IQR Outlier} monitor template with a specified distance threshold of 100. 

Next, we identify a UDF for targeted fuzzing. Given the complexity of the \codefont{solve\_collatz} function, we decide to isolate the corresponding \codefont{solved} transformation. As a result, we isolate a UDF that consumes \codefont{(Int, Iterable[Int])} and produces \codefont{(Int, Int)} outputs.

\subsubsection{Mutations.}
Based on the monitor template and the UDF type signature, \tool identifies the following mutations from Table \ref{table:mutations} and weights them as follows\footnote{Mutations in parentheses are combined to match the required UDF input type.}: 
\begin{itemize}
    \item RandomInteger\\(RandomRecord+TupleElementMutation), 1.0
    \item CollectionConcatenation\\(RandomRecord+TupleElementMutation), 1.0
    \item CollectionElementMutation\\(RandomRecord+TupleElementMutation), 5.0
    \item KeyEnumeration, 0.5
    \item ValueEnumeration, 0.5
    % \item DuplicateKeyGeneration, 0.5
    %  While originally intended, this was not supported due to type and implementation limitations.
    % (It's hard to generate a random iterable of values and would require more composition than currently supported)
    \item DuplicateValueGeneration, 0.5
    
\end{itemize}
 Due to the monitor template's focus on partition runtime skew, \tool decreases the weights of the data skew mutations. At the same time, it increases the weight of \textit{CollectionElementMutation} to encourage fuzzing to explore each item within the \codefont{Iterable[Int]} value.

\subsubsection{Input Seed.} % jason: this is in a different order from other evals
Finally, fuzzing requires a program input seed as a basis for mutations. For simplicity, we create a simple program input seed with following data:
\begin{center}
\begin{tabular}{r}
Program Input\\
\hline
"1" \\
\hline
"2"\\
\hline
"3"\\
\hline
"4"\\
\hline
\end{tabular}
\end{center}
When testing this seed input, \tool finds that no performance skew is exhibited. Furthermore, manual inspection of each element indicates that all integers have relatively short Collatz conjecture sequence lengths, with the longest being a sequence of length 7 for the integer "3".

\subsubsection{Intermediate Input Generation.}
\tool's phased fuzzing approach fuzzes the isolated UDF. It starts by first partially running the program with the provided program input seed to determine an appropriate UDF input seed.
\begin{center}
\begin{tabular}{r}
UDF Input\\
\hline
(1, [1])\\
\hline
(2, [1])\\
\hline
(3, [1])\\
\hline
(4, [1]) \\
\hline
\end{tabular}
\end{center}
Using this UDF input seed and the mutations noted earlier, \tool fuzzes the UDF. After 34 iterations and 30385 ms, it produces a skew-inducing UDF input by applying the \textit{RandomInt} mutation (in combination with \textit{TupleElementMutation} on the tuple key) to alter the bolded record key from "1" to "1497909577":
\todo{Update numbers and results to match new data}
\begin{center}
\begin{tabular}{r}
UDF Input\\
\hline
(\textbf{1497909577}, [1])\\
\hline
(2, [1])\\
\hline
(3, [1])\\
\hline
(4, [1]) \\
\hline
\end{tabular}
\end{center}
"1497909577" has a much longer Collatz conjecture sequence length of 183 numbers which, when combined with the \codefont{solve\_collatz} function, results in significantly longer computation time compared to the remaining records. As a result, \tool has successfully identified a UDF input that produces the desired performance skew.

\subsubsection{Inverse Function.} % jason: different order from other evaluations
As \tool aims to trigger performance skew with program inputs, it converts this UDF input into a program input through the use of an inverse function. \changed{In order to invert lines 3-7 of the \textit{Collatz} program in Figure \ref{fig:collatz_sparkrdd}, we define the following inverse function}:
\input{code/code_collatz_inverse_fn}
% \jason{There's some drawbacks to this inverse function, e.g. it's impossible to reverse a flatMap if there's no common key to regroup records by. I'm not sure it's worth mentioning here though.}
% jason: removed 4/13 since we aren't using prose anymore. Due to existing limitations which require manual intervention to adopt the Prose function into \tool, the process of generating this inverse function takes up to 5 minutes that includes the initialization time for Prose, feeding inputs, and C\# to Scala conversion. 

\subsubsection{Program Input Generation.}
\tool applies this inverse function on the UDF input generated from fuzzing, which produces the following program inputs after 137 ms:
\begin{center}
\begin{tabular}{r}
Program Input\\
\hline
\hline
"4"\\
\hline
"1497909577"\\
\hline
"1"\\
\hline
"3"\\
\hline
\end{tabular}
\end{center}

Finally, \tool uses this input along with \textit{ReplaceSubstring} mutation to fuzz the program inputs for the same performance symptom defined by our existing monitor template. In this case, only one iteration is required  as \tool verifies tests the inverted input, which takes 27180 ms, and finds that it is already sufficient for triggering the desired performance skew symptoms. 
%\jason{See note in approach, we might want to discuss how it's sometimes sufficient to simply convert UDF input -> program input with the inverse function. Alternatively consider an additional extension/evaluation to produce more inputs, e.g. reuse UDF-based seed and run for X minutes to identify new inputs to compare speed against the baseline.}

\subsubsection{Baseline Comparison.}
As a baseline, we also use \tool to directly fuzz the program inputs using our initial seed input as opposed to the improved seed identified through UDF fuzzing and the inverse function. After 58426 iterations and 2668253 ms (almost 45 minutes), the following result is produced:
\begin{center}
\begin{tabular}{r}
Program Input\\
\hline
"1"\\
\hline
"2"\\
\hline
"3"\\
\hline
% A909
% "\includegraphics[width=2mm]{images/9.pdf}4"\\
% \KLNine
% \hline
"3\includegraphics[width=3mm]{images/38-2.png}"\\ 
\hline
\end{tabular}
\end{center}
% Credit goes to Qian for finding a workaroudn to include the unicode character - it should be kayah li 9 (unicode U+A909). Jason was otherwise unable to get the Google suggestion of \\usepackage[utf8x]\{inputenc\} as well as trying a different unicode-compatible compiler (I tested XeLaTeX with no luck)}. Thank you Qian!
% Update 4/11: Changing results, we now have Limbu Digit 3 and N'Ko digit 8
% ᥉߈
% "3\includegraphics[width=3mm]{images/38-2.png}"\\ 
% https://en.wikipedia.org/wiki/Limbu_script
% https://en.wikipedia.org/wiki/N'Ko\_script



While the final record does not immediately appear to be numeric, manual investigation revealed that the first character actually corresponds to "9" in the Kayah Li alphabet\footnote{https://en.wikipedia.org/wiki/Kayah\_Li\_alphabet} and is considered a valid integer string in Scala.

% Results spreadsheet for Collatz https://docs.google.com/spreadsheets/d/1oK1u_iZckc9R10DlPgW_JNW_2OYJu0L6gFO8jxFmiW4/edit?usp=sharing
%metrics: Speedup of phased vs naive fuzzing. Speedup of improved input seed [evaluation only, less significant]. Improvement in fuzzing accuracy. 
\begin{table}[t]
{    %\nocaptionrule
    \centering
    % original scale 0.68
        \scalebox{0.8}{\input{tables/collatz_results}}
        
		
    \vspace{1ex}
    \caption{Fuzzing times and number of iterations for the Collatz case study. \textit {Phased Fuzzing} represents the entire \tool approach and includes \textit{UDF Fuzzing}, time spent applying the inverse function to the result of \textit{UDF Fuzzing}, and \textit{Program Fuzzing with Improved Seed}.}
    \label{table:collatz_results}
} 
% 		\vspace{-3ex}
%\vspace{-6ex}
\end{table}

\subsubsection{Results.}
% \changed{
\changed{The results for both \tool and baseline are summarized in Table \ref{table:collatz_results}. Compared to the baseline, \tool leads to a 46X speedup in workload generation speed if the inverse function is predefined. Including an upper bound of 5 minutes overhead for identifying an inverse function, \tool achieves almost 7.5X speedup compared to the baseline. When fuzzing the original program, using an improved input seed derived from UDF fuzzing results in 98X speedup compared to fuzzing with the original input seed.}

\changed{Furthermore, the use of the improved input seed requires far fewer iterations compared to the original input seed. \tool is able to produce a symptom-triggering input in a single iteration, 1/58426 the number of iterations required by the baseline approach. This is possible because \tool directly targets the isolated UDF and is able to generate an intermediate input which successfully triggers the target symptom in 34 iterations, less than 0.06\% the number of iterations required for the baseline to produce inputs for the full program. This contrast demonstrates the challenges of fuzzing paths deep inside programs and the potential for more accurate fuzzing mutations through program slicing. In particular, \tool's type-aware approach is able to address the \textit{Collatz} program's expectation of numerical inputs while the baseline is restricted to string-based mutations.}

% Original ASPLOS: The results for both \tool and baseline are summarized in Table \ref{table:collatz_results}. Comparing this baseline approach to \tool's phased fuzzing, using \tool leads to a 46X speedup in workload generation speed if the inverse function is predefined. Including an upperbound of 5 minutes overhead for identifying an inverse function, \tool achieves almost 7.5X speedup compared to the baseline. When fuzzing the original program, using an improved input seed derived from UDF fuzzing results in 98X speedup compared to fuzzing with the original input seed. Furthermore, the improved input seed produces 58425X improvement in fuzzing accuracy compared to the original input seed. In other words, baseline setup produces over 58425 inputs before reaching the required performance symptom whereas \tool does the same in 1 iteration. Finally, \tool uses skew-inspired mutations to fuzz the isolated UDF with 1717X better accuracy compared to fuzzing the full program, thus highlighting the challenge of fuzzing paths deep inside programs and the potential for more accurate fuzzing mutations through program slicing. 
%\jason{Could potentially use more interpretation/significance discussion here if time permits}.

==> case_studies/old/case_study_dept_old.tex <==

\subsection{Case Study: DeptGPAsMedian}
\label{sec:case_study_deptgpas}
\changed{\jason{This entire section is new w.r.t. ASPLOS submission}}
% \subsubsection{Program and Symptom}
% \noindent{\bf Program description} TODO: Program, origin(?) (description + code), origins, 
% % note: input/output can be derived from description.
\subsubsection{Program Definition.}
The \textit{DeptGPAsMedian} program is modified from \cite{teoh:socc:flowdebug} and is shown in Figure \ref{fig:code_dept}. Given a string dataset with lines in the format \textit{"studentID,courseID,grade"}, the program first computes each course's average GPA. Next, it groups each average GPA according to the course's department and computes each department's median average course GPA.

\begin{figure}[t]
\centering 
\input{code/code_deptgpamedian_program}
\vspace{-2ex}
\caption{The \textit{DeptGPAsMedian} program implementation in Scala which calculates the median of average course GPAs within each department. \jason{I'm not sure this figure is truly necessary, it adds little value compared to the text description.}}
\label{fig:code_dept}
\end{figure}
% \noindent{\bf Symptom + Location} What is the symptom to be reproduced? e.g., 
% In one execution, the developer observed one partition taking X time longer than others in a particular stage. However, they are no longer able to access this particular input. 
% [alts: they observed a bug report without data, or want to see if there's a situation here X can occur]

% Looking at the Spark execution graph, they suspect the issue to be in the UDF that does X. In particular, this UDF has an input schema of X. (not sure if schema necessary). 
\subsubsection{Symptom.}
\todo{Make sure subject developer (name/reference) matches tone in other case studies}.
The developer believes that data skew can pose a problem in the \textit{DeptGPAsMedian} program, but isn't sure how to demonstrate this with a valid dataset. Nonetheless, they know that such data skew can be identified by an imbalance in the number of records that map to each department in the second aggregation of the program, as determined by the \textit{groupByKey} operator. 

\subsubsection{Input Seed.}
The developer has previously generated a 40-partition, 2.8MB example dataset consisting of 5,000 records per partition. The dataset includes five departments, 20 courses per department, and 200 unique students. While this dataset is sufficient for running the \textit{DeptGPAsMedian} program, it does not exhibit any sort of data skew.

% [snippet of program input]
% [UDF snippet if necessary]

% \noindent{\bf Initial seed} The user first [hand-generates, samples, derives] an initial input as shown below: [figure]. However, running their program with this input does not reproduce the symptom. To investigate further, they hope to use \tool to generate an appropriate dataset.
% \noindent{\bf Monitor Template} How the skew is translated to a template. 
\subsubsection{Monitor Template Definition.}
The developer plans to use \tool to generate a data skew-inducing input dataset. First, they define an appropriate monitor template by using  the \textit{Shuffle Read Records} metric with a \textit{Next Comparison} template and ratio threshold of \textit{100.0}, indicating that the largest partition must read at least 100x the number of shuffle records as the next largest partition.
% \noindent{\bf Mutations} Which mutations and weights, derived from UDF + Monitor Template. 
% Need to specify two additional user settings here too for the sake of evaluation.

% plan: justify the increased duplication factor. adjust the mutation weight.
\subsubsection{Mutations.}
The developer also expects relatively small intermediate partitions as there are 100 unique course averages across 40 partitions. To enable \tool to better generate data skew, they increase the maximum duplication factor to 5x to allow for more significant dataset mutations. \tool then uses both the data skew symptom definition and this hint to generate the following mutations and weights for the input of type \textit{(String, Double)}:

\begin{itemize}
    \item ReplaceSubstring\\(RandomRecord+TupleElementMutation), 1.0
    \item RandomDouble\\(RandomRecord+TupleElementMutation), 1.0
    \item KeyEnumeration, 1.0
    \item ValueEnumeration, 1.0
    \item DuplicateKeyGeneration(5.0), 5.0
    \item DuplicateValueGeneration(5.0), 5.0
\end{itemize}
% From execution logs: GenericRandomKeyMutationFn() -> 1.0, GenericKeyEnumerationMutationFn() -> 1.0, GenericRandomValueMutationFn() -> 1.0, GenericKeyDuplGenMutationFn(5.0) -> 5.0, GenericValueDuplGenMutationFn(5.0) -> 5.0, GenericValueEnumerationMutationFn() -> 1.0

Due to the monitor template's focus on data skew, \tool increases the weights of the the data skew-oriented \textit{DuplicateKeyGeneration} and \textit{DuplicateValueEnumeration} mutations. 


% \subsubsection{\tool running}
\subsubsection{Inverse Function.}
As a final input requirement, the developer must define an inverse function to map the \textit{groupByKey} inputs to \textit{DeptGPAsMedian} program inputs. They note that each \textit{(dept, avg)} pair must correspond to a unique course ID due to the previous aggregation by course, and that the student ID value in the full program input is irrelevant. As \tool does not always require the inverse function to be exact, the developer also chooses to approximate reversing the average aggregation by generating a single record per course. With this in mind, they define the following function:

\input{code/code_deptgpamedian_inverse_fn}

\subsubsection{Intermediate Input Generation.}
Now that all input requirements are satisfied, \tool can begin running. It uses the provided input to execute the \textit{DeptGPAsMedian} program up until the \textit{groupByKey} operator and generate an intermediate input seed after 2282 ms:

% head /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220315/deptgpaquartiles_nxtcmp100_dupe5/seeds/udf/0_text/part-00000
\begin{center}
\begin{tabular}{r}
\textit{groupByKey} Input\\
\hline
("Physics", 2.355523672883788)\\
\hline
("STATS", 2.3666507860886137)\\
\hline
("Physics", 2.3563752276867036)\\
\hline
("MATH", 2.369141755062681)\\
\hline
...\\
\hline
\end{tabular}
\end{center}

% \noindent{\bf Phased Fuzzing} Paragraph 1: The UDF Fuzzing results - example snippets of intermediate seed input, mutations applied, output, time taken, number of iterations.
% /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220315/deptgpaquartiles_nxtcmp100_dupe5/intellij_deptgpaquartiles_phased_with_reverse.log

Starting with this input, \tool applies the earlier mutations to trigger the target data skew symptom. After 1519 iterations and 259205 ms, it generates such an input by applying the \textit{DuplicateKeyGeneration} to a previously modified input which results in a \textit{Next Comparison} ratio of over 353x. As the monitor template's threshold is 100x, this result is determined to trigger the desired data skew. Upon manual investigation, we find that this mutation increased the number of "EE" records in intermediate partition #17 from 1111 to 6466 (an increase of approximately 4.82x), which then led to a total of 6711 shuffle read records on the partition to which "EE" records are assigned compared to the next largest partition with 19 records. 
% Note: snippet not necessary here as it takes up too much space to properly illustrate, and is better summarized in plain text. A small snippet can be shown in the input seed, if anything (but plain text is still sufficient I think).

% Paragraph 2: Result of applying the inverse function to produce a program input.
\subsubsection{Program Input Generation.}
Next, \tool generates an input seed by applying the inverse function:
% head /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220315/deptgpaquartiles_nxtcmp100_dupe5/seeds/e2e/0_text/part-00000
\begin{center}
\begin{tabular}{r}
\textit{DeptGPAsMedian} Input\\
\hline
"42,Physics0,2"\\
\hline
"42,STATS40,2"\\
\hline
"42,Physics80,2"\\
\hline
"42,MATH120,2"\\
\hline
...\\
\hline
\end{tabular}
\end{center}

% Paragraph 3: Using result as seed input for end-to-end fuzzing - example snippet of output, time taken, number of iterations. Any other useful breakdown numbers too. [if the input only requires one iteration, this can be kept short]

% /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220315/deptgpaquartiles_nxtcmp100_dupe5/intellij_deptgpaquartiles_phased_with_reverse.log
Finally, \tool tests this input to the full \textit{DeptGPAsMedian} program. After the program runs for 638 ms, \tool finds that it triggers the data skew symptom defined by the developer with a \textit{Next Comparison} ratio score of over 350.

% Paragraph 4: Baseline comparison: snippet of output if applicable, time taken, number of iterations. [if there's no result, this can be shortened too]
% /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220224/deptgpaquartile_recread/nextcmp_1000_dupe50_baseline/
\subsubsection{Baseline Comparison.}
We also test \tool using the original provided input as a baseline seed. However, no satisfying inputs were generated after running for 4 hours; the maximum \textit{Next Comparison} ratio score increased from an in initial 3.0 to about 6.68, while the target ratio was specified as 100.0. 

% Concluding Paragraph Summarized findings for case study.
\subsubsection{Results.}
All results for the \textit{DeptGPAsMedian} program are summarized in Table \ref{table:deptgpamedian_results}. \tool produces an input which triggers the desired symptom in under 4.5 minutes, with 1519 iterations of intermediate input generation. Furthermore, the program input produced by applying the inverse function is found to require no additional modification to continue producing the desired symptom. In comparison, the baseline approach did not produce any results after four hours and 21,575 iterations. At the end of these four hours, the largest \textit{Next Comparison} ratio observed was less than 7\% of the target threshold defined by the monitor template.

\tool's better performance can largely be attributed to its ability to target its mutations at intermediate records for the \textit{groupByKey} operation, after the first aggregation to compute average course GPAs. In particular, the \textit{DuplicateKeyGeneration} and \textit{DuplicateValueGeneration} mutations combined with the provided inverse function are able to generate many new courses at once, which then leads to a noticeable increase in the number of shuffle read records which is used as the primary metric in the monitor template for this case study. In contrast, the baseline modifies at most a single input record with each iteration. Due to the initial aggregation, such mutations are limited in effectiveness and manage to only slighty increase the number of shuffle read records if the \textit{courseID} field is changed to a new, unique value.

\jason{Plot data exists, but comparing ~5min vs 4 hours makes for a terrible graph (similar to Stock graph) so it is omitted for now.}
% Upon closer investigation, we observe that the baseline approach faces two key challenges. First, its string-based mutations fail to account for the fields and data types required by the input: only 3 of the 8 comma-separated fields are used in the \StockProgramName program, and one of these must be numeric. As a result, many of the iterations yield inputs that are either invalid or functionally identical to existing ones.

% Second, the baseline approach has difficulty exploiting the collection-based properties of values in the \maxProfitsRDD RDD. As \maxProfitsRDD comes after a \textit{groupByKey} operation, the baseline's single-record mutation can affect at most a single element within the value of any given \maxProfitsRDD record. 

% \tool is able to overcome the first challenge through its knowledge of the data types that go into the \maxProfitsRDD RDD. Furthermore, its collection-based mutations enable \tool to overcome the second challenge by generating more diverse inputs that are more likely to improve affect the partition counter accumulators defined in \StockProgramName and thus improve the metric associated with the desired target symptom.



\begin{table}[t]
{    %\nocaptionrule
    \centering
    % original scale 0.68
        \scalebox{0.8}{\input{tables/deptgpamedian_results}}
        
    \vspace{1ex}
    \caption{Fuzzing times and number of iterations for \textit{DeptGPAsMedian} program. *Baseline evaluation timed out and was unable to trigger the desired symptom. \jason{See note in Stock table.}}
    \label{table:deptgpamedian_results}
} 
% \vspace{-3ex}
% \vspace{-6ex}
\end{table}
% Can't have a comparison, since baseline didn't work at all.
% Compared to the baseline approach, using \tool leads to an overall \todo{X} speedup while dedicating \todo{X2\%} of its time to fuzzing the intermediate UDF. The improved input seed generated from UDF fuzzing resulted in \todo{Y} speedup and required \todo{less than Z\%} iterations compared to the baseline. 


==> case_studies/old/case_study_stocks_old.tex <==
\subsection{Case Study: StockBuyAndSell}
\changed{\jason{Round 2 - rewrote almost everything to simplify/focus on key points and definitions.}}
\newcommand{\StockProgramName}{\textit{StockBuyAndSell}\xspace}
\newcommand{\maxProfitsRDD}{\textit{maxProfits}\xspace}
\soulregister{\StockProgramName}{7}
\soulregister{\maxProfitsRDD}{7}
% \subsubsection{Program and Symptom}
% \noindent{\bf Program description} TODO: Program, origin(?) (description + code), origins, 
% % note: input/output can be derived from description.
\subsubsection{Program Definition.}
The \StockProgramName program is based on the LeetCode \textit{Best Time to Buy And Sell Stock III} coding problem \cite{leetcode-buy-and-sell-iii}. Using a dataset of comma-separated strings in the form \textit{"Symbol,Date,Open,High,Low,Close,Volume,OpenInt"}, the \StockProgramName calculates the maximum achievable profit with at most three transactions by grouping closing prices by stock symbol and sorting within each symbol. For each such ordered group of prices, a Scala adaptation of LeetCode user \textit{peetleetcode}'s solution \cite{leetcode-buy-and-sell-iii-peetleetcode-solution} is applied to compute the optimal profit . The program implementation is shown in Figure \ref{fig:code_stock}, where the \maxProfitsRDD variable is the result of applying the profit calculation for each group.
% https://leetcode.com/problems/best-time-to-buy-and-sell-stock-iii/
% https://leetcode.com/problems/best-time-to-buy-and-sell-stock-iii/discuss/39608/A-clean-DP-solution-which-generalizes-to-k-transactions
\begin{figure}[t]
\centering 
\input{code/code_stockbuysell_program}
\vspace{-2ex}
\caption{The \StockProgramName program implementation in Scala which calculates maximum achievable profit with at most three transactions (\maxProfitsRDD, lines 16-40), for each stock symbol. To support a user-defined metric, a Spark accumulator (line 2) is defined and updated via a custom iterator (lines 42-51).}
\label{fig:code_stock}
\end{figure}


\subsubsection{Symptom.}
Rather than relying on performance metrics, the developer wishes to explore what inputs might frequently increase the maximum observed profit at any point within their algorithm. More specifically, their specific interest is found in the UDF that generates the \maxProfitsRDD RDD which takes as input records of type \textit{(String, Iterable[Double])}. They hope to use \tool to generate an input that meets this condition many times for a subset of inputs. 
\gulzar{I am a little confuse. Does this example demonstrate perfgen's performance fuzzing or just normal coverage based fuzzing? Since the goal is to amplify a certain behavior?}
\subsubsection{Input Seed.}
As an input seed, the developer uses an existing Kaggle dataset posted by user \textit{borismarjanovic} \cite{Kaggle-Stock-Data-Marjanovic2017}. As the data is originally separated by stock symbol and does not contain that information within each record, preprocessing is applied to match the \StockProgramName schema. Furthermore, the dataset is far larger than necessary for demonstrating the desired symptom, so the developer selects a subset by sampling 1\% of data from the 20 largest stock symbols. The final input seed consists of 2,389 records across 20 partitions, totaling 244KB of data in total.
% https://www.kaggle.com/borismarjanovic/price-volume-data-for-all-us-stocks-etfs 


% [snippet of program input]
% [UDF snippet if necessary]

\subsubsection{Monitor Template Definition.}
As \tool does not provide out-of-the-box support for capturing branch execution counts within each partition, the developer utilizes the Spark Accumulator API \footnote{https://spark.apache.org/docs/2.4.4/rdd-programming-guide.html\#accumulators} to track the number of times that the \textit{maxProfit} variable is increased within each partition (lines 2, 33-34, 42-51). The developer then uses this accumulator to define a custom metric for these partition-level metrics, which is then passed to a \textit{Next Comparison} monitor template with a target ratio of 5.0. 

\subsubsection{Mutations.}
The developer recognizes that the stock symbol values do not directly affect their metric of interest and chooses to disable mutations that affect the key values of the \maxProfitsRDD RDD. Furthermore, \tool recognizes that the earlier \textit{groupByKey} operation restricts the keys to be unique within \maxProfitsRDD. As a result, only two mutations are generated:

\begin{itemize}
    \item CollectionConcatenation\\(RandomRecord+TupleElementMutation), 1.0
    \item CollectionElementMutation\\(RandomRecord+TupleElementMutation+RandomDouble), 5.0
\end{itemize}
% From execution logs: GenericIterableValueMutationFn() -> 5.0, GenericIterableValueDuplMutationFn(2) -> 1.0

Due to the use of a custom metric, \tool does not adjust the weights of each mutation beyond the default values.


\subsubsection{Inverse Function.}
To generate \StockProgramName inputs from the \maxProfitsRDD inputs, the developer manually implements a function which first assigns a chronological date to each stock price. 
As the \StockProgramName program does not make use of the values for \textit{Open,High,Low,Volume} or \textit{OpenInt}, the developer also specifies arbitrary values for each unused field. Finally, all values are joined into the original comma-separated format required by \StockProgramName.

\input{code/code_stockbuysell_inverse_fn}

\subsubsection{Intermediate Input Generation.}
Using the provided input seed, \tool first generates an input to the \maxProfitsRDD RDD:

% head /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220315/stock_nxtcmp5_partition_sampled_phased_gt-only/seeds/udf/0_text/part-00000 /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220315/stock_nxtcmp5_partition_sampled_phased_gt-only/seeds/udf/0_text/part-00001 /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220315/stock_nxtcmp5_partition_sampled_phased_gt-only/seeds/udf/0_text/part-00002
% There's very few lines per file so you need multiple
\begin{center}
\begin{tabular}{r}
\maxProfitsRDD Input\\
\hline
(intc,MapLike.DefaultValuesIterable(0.01592, 0.03216,...)\\
\hline
(jnj,MapLike.DefaultValuesIterable(0.4801, 0.9116,...)\\
\hline
...\\
\hline
\end{tabular}
\end{center}

% /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220315/stock_nxtcmp5_partition_sampled_phased_gt-only/intellij_stockbuyandsell_phased.log
\tool then applies mutations to this input to increase the \textit{Next Comparison} ratio as specified by the monitor template. After 205084 ms and 4775 trials, it produces a satisfying input from applying the \textit{CollectionElementMutation} to a previously mutated input which results in a \textit{Next Comparison} ratio of approximately 5.08. More specifically, the input contains a partition with a modified price list that triggers the desired if-branch 330 times, compared to the next closest partition which triggers the same branch only 65 times.
% 257 commas in part-00015 vs 1642 in part-00010 (-1 for the key-value comma)
% [PartitionsMutationFnFuzzer: 19:09:52] Full partition metrics (sorted) (20): 0,0,0,0,0,0,0,30,32,34,42,43,45,49,52,54,63,64,65,330

\subsubsection{Program Input Generation.}
\tool applies the previously defined inverse function to the symptom-triggering \maxProfitsRDD input to produce an input seed for the \StockProgramName program. After running this input for 146 ms, \tool finds that it triggers the specified \textit{Next Comparison} template definition with the same ratio identified while generating inputs for the intermediate \maxProfitsRDD RDD.
% Not showing snippet as it doesn't help here...

% \todo{Fill in the result - need a summary?}

% Paragraph 4: Baseline comparison: snippet of output if applicable, time taken, number of iterations. [if there's no result, this can be shortened too]
% TODO: source/log file path
\subsubsection{Baseline Comparison.}
For comparison, we also evaluate the \StockProgramName program using initially provided input seed as a starting point for workload generation. After 4 hours, no inputs were generated that triggered the symptom defined by the previously defined monitor template. At the end of these 4 hours, the observed \textit{Next Comparison} ratio metric had increased from an initial 1.85 to a peak of 2.52 - far lower than the desired 5.0 threshold. 

% Concluding Paragraph Summarized findings for case study.
\subsubsection{Results.}
% data in spreadsheet: https://docs.google.com/spreadsheets/d/15w-uDdhQl9u_8R5c8foRGar_mP1npDIwxiOW8PZLkMQ/edit#gid=1535004788
\StockProgramName evaluation results are summarized in Table \ref{table:stockbuysell_results}, with the progress of the best observed \textit{Next Comparison} ratios plotted in Figure \ref{plot:stockbuysell}. \tool is able to generate a symptom-triggering input to the \StockProgramName program in slightly under 3.5 minutes, and requires 4775 iterations of intermediate input generation. Using the inverse function defined earlier, the generated intermediate input seed is converted to a \StockProgramName input that triggers the target symptom without any additional modifications. In contrast, the baseline is unable to trigger the desired symptom after four hours and 40,010 iterations of generating inputs. At the end of this period, the baseline is able to achieve a maximum \textit{Next Comparison} ratio of approximately 2.5 - roughly half of the target threshold of 5.0 defined in the monitor template. 

Upon closer investigation, we observe that the baseline approach faces two key challenges. First, its string-based mutations fail to account for the fields and data types required by the input: only 3 of the 8 comma-separated fields are used in the \StockProgramName program, and one of these must be numeric. As a result, many of the iterations yield inputs that are either invalid or functionally identical to existing ones.

Second, the baseline approach has difficulty exploiting the collection-based properties of values in the \maxProfitsRDD RDD. As \maxProfitsRDD comes after a \textit{groupByKey} operation, the baseline's single-record mutation can affect at most a single element within the value of any given \maxProfitsRDD record. 

\tool is able to overcome the first challenge through its knowledge of the data types that go into the \maxProfitsRDD RDD. Furthermore, its collection-based mutations enable \tool to overcome the second challenge by generating more diverse inputs that are more likely to improve affect the partition counter accumulators defined in \StockProgramName and thus improve the metric associated with the desired target symptom.

\begin{table}[t]
{    %\nocaptionrule
    \centering
    % original scale 0.68
        \scalebox{0.8}{\input{tables/stockbuysell_results}}
        

    \vspace{1ex}
    \caption{Fuzzing times and number of iterations for \StockProgramName. *Baseline evaluation timed out and was unable to trigger the desired symptom. \jason{Compared to Collatz, I also included stat for intermediate seed comp and inverse function application. The totals don't perfectly add up due to other CPU cycles (logging)}}
    \label{table:stockbuysell_results}
} 
% \vspace{-3ex}
% \vspace{-6ex}
\end{table}

% \input{plots/time-series-fuzzing}
\begin{figure*}[t]
    \centering
% https://tex.stackexchange.com/questions/75449/specifying-the-width-and-height-of-a-tikzpicture
% \resizebox{width}{height}{object}
% \resizebox{\textwidth}{!}{%
    \begin{tikzpicture}
    \begin{axis}[title=\textbf{StockBuyAndSell},xmin=0,xmax=240,xmode=linear,ymax=5.5,width=\textwidth]
       \input{plots/time-series-subplots/stockbuysell_timeseries}
    \end{axis}
    \end{tikzpicture}
    
    \caption{\todo{Caption and resize, if we keep this figure. Jason isn't sure it's very valuable given the scale.}}
% }
\label{plot:stockbuysell}
\end{figure*}

==> case_studies/old/case_study_wordcount_old.tex <==
\subsection{Case Study: WordCount}
\changed{\jason{This entire section is new w.r.t. ASPLOS submission}}
% \subsubsection{Program and Symptom}
% \noindent{\bf Program description} TODO: Program, origin(?) (description + code), origins, 
% % note: input/output can be derived from description.
\todo{Planning to rerun this one, so many parts are intentionally left as TODOs. There are challenges w.r.t. consistency and scale for the symptom.}
\subsubsection{Program Definition.}
The WordCount program comes from\todo{cite spark examples} and is shown in Figure \todo{ref code figure}. The program takes as input a string dataset of space-separated words and outputs pairs consisting of each unique word and the number of its occurrences. \todo{Jason: considering changing whitespace separator, update here if so}.

% \noindent{\bf Symptom + Location} What is the symptom to be reproduced? e.g., 
% In one execution, the developer observed one partition taking X time longer than others in a particular stage. However, they are no longer able to access this particular input. 
% [alts: they observed a bug report without data, or want to see if there's a situation here X can occur]

% Looking at the Spark execution graph, they suspect the issue to be in the UDF that does X. In particular, this UDF has an input schema of X. (not sure if schema necessary). 
\subsubsection{Symptom.}
Suppose a Spark developer observes in the Spark History Server logs that a prior instance of WordCount ran for an unusually long time \todo{better motivate this start}. The developer wants to investigate this particular execution to understand why this is the case, but unfortunately it has been many days since the original execution and the data is no longer available. However, they are able to observe through the logs that there are significant differences in processing times for Spark executors in the first stage of the 2-stage WordCount program. Based on their knowledge of the program, they suspect this to be due to the \textit{reduceByKey} operator.

\subsubsection{Input Seed.}
As an initial investigation, the developer tries the WordCount program using an existing dataset that they already have on hand: the Large Movie Review Dataset \todo{cite (comments)}. The developer decides to use 11 files under the positive training samples which start with "1000*", which consists of 2,564 words and 44KB. Each file consists of a single movie review. However, this small test dataset does not exhibit any unusual performance when passed through the WordCount program.
% http://ai.stanford.edu/~amaas/data/sentiment/ - cite has bib to link to.

% [snippet of program input]
% [UDF snippet if necessary]

% \noindent{\bf Initial seed} The user first [hand-generates, samples, derives] an initial input as shown below: [figure]. However, running their program with this input does not reproduce the symptom. To investigate further, they hope to use \tool to generate an appropriate dataset.
% \noindent{\bf Monitor Template} How the skew is translated to a template. 
\subsubsection{Monitor Template Definition.}
In order to better understand what may have caused the previous performance skew, the developer turns to \tool. The developer first concretely defines the performance skew symptom they wish to reproduce by utilizing the \textit{Runtime} metric with the predefined \textit{Skewness} template and upper threshold of \textit{2.0} \todo{optional footnote on value selection, see comments}.
% typically 1.0 is already considered an outlier, so 2.0 could be considered extreme. However, the smaller sample set makes things a bit more variable here.
% \noindent{\bf Mutations} Which mutations and weights, derived from UDF + Monitor Template. 
% Need to specify two additional user settings here too for the sake of evaluation.
\subsubsection{Mutations.}
In addition to this symptom definition, the developer also adjusts two settings in \tool before it generates mutations. First, they restrict \tool so that values in the key-value pairs of the \todo{reduceByKey} inputs are never modified, as these should always be "1" according to program definition. Second, they increase the maximum duplication factor up to 100x as the initial input partition sizes are fairly small. Combining the symptom definition with these two user-provided settings, \tool identifies the following set of mutations and weights for the intermediate inputs of type \textit{(String, Int)}: 
\begin{itemize}
    \item ReplaceSubstring\\(RandomRecord+TupleElementMutation), 1.0
    \item KeyEnumeration, 1.0
    \item DuplicateKeyGeneration, 1.0
\end{itemize}
% From execution logs:
% GenericRandomKeyMutationFn() -> 1.0, 
% GenericKeyDuplGenMutationFn(100.0) -> 1.0, 
% GenericKeyEnumerationMutationFn() -> 1.0


\todo{Revisit weights after re-evaluation. See comments.}
% This should be weighted and I'll need to do a new evaluation. After that, discuss why things are weighted. Plan right now is to have DuplicateKeyGen weighted higher. See comments.}
% I'm actually not 100\% sure how this will work, especially given how Collatz uses the same metric and similar template yet downweights keyenum and duplicatekeygen. Perhaps I should justify it according to the data types too (since Collatz has K+[many-val], and WC has K+immutable-val) - it makes more sense that DuplicateKeyGen has more impact than KeyEnum (which isn't really repeatable) or RandomString (which affects one record at a time).}
% 

% \subsubsection{\tool running}
% \noindent{\bf{Inverse Function prereq}} In order to utilize \tool, developer must provide a mapping from UDF input to Program input. In the case of Collatz, the user utilizes Prose [cite] in combination with their knowledge of Spark operator semantics to define the following function. (potential callback to how the inverse functions do not have to be perfect, and that sometimes multiple may exist).
\subsubsection{Inverse Function.}
As a final step before \tool attempts to reproduce the desired performance symptom, the developer defines an inverse function to convert the \textit{reduceByKey} inputs into program inputs. While the \textit{reduceByKey} inputs are pairs of each word occurrence and a '1', there is no information as to how the grouping or ordering of these words in the original program input. As a result, the Spark developer arbitrarily chooses to assign 50 words into each line as follows:

\input{code/code_wordcount_inverse_fn}

\todo{optional callback to the inverse function requirements, in particular that there may be many options and it doesn't have to be perfect}.

\subsubsection{Intermediate Input Generation.}
Now that all input requirements are satisfied, \tool begins by testing the provided seed input. Like the developer, it finds that there is no pre-existing performance skew and proceeds to isolate the \textit{reduceByKey} operation. First, \tool runs the WordCount program with the provided seed up until the UDF inputs which consist of each word and a "1":

\begin{center}
\begin{tabular}{r}
UDF Input\\
\hline
("Homelessness", 1)\\
\hline
("(or", 1)\\
\hline
("Houselessness", 1)\\
\hline
("as", 1)\\
\hline
...\\
\hline
\end{tabular}
\end{center}

% \noindent{\bf Phased Fuzzing} Paragraph 1: The UDF Fuzzing results - example snippets of intermediate seed input, mutations applied, output, time taken, number of iterations.

Next, \tool applies the aforementioned mutations on this UDF input to generate new UDF datasets while monitoring for the desired performance symptoms. After \todo{X} iterations and \todo{Y} ms, \tool identifies a skew-inducing input by applying \todo{Mutation-history} to produce an intermediate dataset where \todo{description of result, Optional result snippet, if possible}. 

% Paragraph 2: Result of applying the inverse function to produce a program input.
\subsubsection{Program Input Generation.}
To map these findings back to inputs for the entire WordCount program, \tool applies the inverse function to produce a new program input. The resulting input consists of \todo{Calculate # of lines and how many show up in modified partition}. 

% Paragraph 3: Using result as seed input for end-to-end fuzzing - example snippet of output, time taken, number of iterations. Any other useful breakdown numbers too. [if the input only requires one iteration, this can be kept short]

Finally, \tool uses this input along with the \textit{ReplaceSubstring} mutation to generate program inputs that satisfy our monitor template. It finds that the original input \todo{Fill this in after re-evaluating, it's possible there's only one iteration required here. Include time taken and number of trials if necessary}.

% Paragraph 4: Baseline comparison: snippet of output if applicable, time taken, number of iterations. [if there's no result, this can be shortened too]
\subsubsection{Baseline Comparison.}
As a baseline, we also test using \tool to directly fuzz the program inputs without targeting the UDF. After \todo{Results: iterations and time}, \todo{Result: findings - probably that some rare occurrence was found but testing revealed that this was not a consistently reproducible performance behavior.}


% Concluding Paragraph Summarized findings for case study.
\subsubsection{Results.}
All results for the \textit{WordCount} program are summarized in Table \todo{ref}. Compared to the baseline approach, using \tool leads to an overall \todo{X} speedup while dedicating \todo{X2\%} of its time to fuzzing the intermediate UDF. The improved input seed generated from UDF fuzzing resulted in \todo{Y} speedup and required \todo{less than Z\%} iterations compared to the baseline. The progress for both executions towards generating the target symptom is shown in Figure \todo{Plot progress time series}, with \todo{Description}. \todo{Takeaway, e.g., highlighting challenge of fuzzing paths deep inside program and/or potential for more accurate fuzzing mutations through program slicing}. 

 

==> code/code_airport_scan.tex <==
\begin{minipage}{\linewidth}
\begin{lstlisting}[language=Scala]
// number of minutes elapsed between two times
def getDiff(arr: String, dep: String): Int = {
  val arr_min = arr.split(":")(0).toInt * 60 + arr.split(":")(1).toInt
  val dep_min = dep.split(":")(0).toInt * 60 + dep.split(":")(1).toInt
  if(dep_min - arr_min < 0){
    return dep_min - arr_min + 24*60
  }
  return dep_min - arr_min
}
  
val pairs = input.map { s =>
  val tokens = s.split(",")
  val dept_hr = tokens(3).split(":")(0)
  val diff = getDiff(tokens(2), tokens(3))
  val airport = tokens(4)
  ((airport, dept_hr), diff)
}
val result = input.reduceByKey(_+_).collect()
\end{lstlisting}
\end{minipage}

==> code/code_commute.tex <==
\begin{minipage}{\linewidth}
\begin{lstlisting}[language=Scala]
val trips = inputs.map { s: String =>
  val cols = s.split(",")
  val distance = cols(3).toInt
  val time = cols(4).toInt
  val speed = distance / time
  if (speed > 40) {
    ("car", speed)
  } else if (speed > 15) {
    ("public transportation", speed)
  } else {
    ("bicycle", speed)
  }
}
val result = trips.aggregateByKey((0L, 0))(
  {case ((sum, count), next) => (sum + next, count+1)},
  {case ((sum1, count1), (sum2, count2)) => (sum1+sum2,count1+count2)},
).mapValues({case (sum, count) => 
  sum.toDouble/count}
).collect()
\end{lstlisting}
\end{minipage}

==> code/code_dupl_key_mutation.tex <==
\begin{lstlisting}[language=Scala]
def appendSameKey[K,V](input: RDD[(K, V)], proportion: Double = 0.10): RDD[(K, V)] = {
    val (key, value) = input.sample(1) // sample one record.
    val numRecordsToAdd = input.count() * proportion
    val newRecords = (1 to numRecordsToAdd).foreach(idx => {
        // create new records with the same key but new values.
        (key, newValue()) 
    })
    // append new records to produce new RDD.
    return input.union(sc.parallelize(newRecords))
}
\end{lstlisting}

==> code/code_example_a.tex <==
%%%%%%%%%%%%%%%%%%%%% Example Code Figure%%%
\begin{figure*}[t]
 \begin{subfigure}[t]{0.49\linewidth}
 \begin{lstlisting}
val log = "s3n://xcr:wJY@ws/logs/weather.log" 
val input :RDD[String] = new SparkContext(sc).textFile(log) 

val split = input.flatMap{ s:String => 
   val tokens = s.split(",") 
   // finds the state for a zipcode
   var state = zipToState(tokens(0))
   var date = tokens(1)
   // gets snow value and converts it into millimeter
   val snow = convertToMm(tokens(2)) 
   //gets year
   val year = date.substring(date.lastIndexOf("/")) 
   // gets month / date	
   val monthdate= date.substring(0,date.lastIndexOf("/")) 
 	 List[((String,String),Float)](   
			((state , monthdate) , snow) , 
			((state , year)  , snow)
		)
}
//Delta between min and max snowfall per key group
val deltaSnow = split
 .groupByKey()
 .mapValues{ s: List[Float]  => 
   s.max - s.min
}
deltaSnow.saveAsTextFile("hdfs://s3-92:9010/")
def convertToMm(s: String): Float = {
  val unit = s.substring(s.length - 2)
  val v = s.substring(0, s.length - 2).toFloat
  unit match {
   case "mm" => return v
   case _ => return v * 304.8f
   }
}
\end{lstlisting}
\vspace{-2ex}
\caption{Original Example 1}
\label{code_example_a}
\end{subfigure}
%
 \begin{subfigure}[t]{0.49\linewidth}
 \begin{lstlisting}
val log = "s3n://xcr:wJY@ws/logs/weather.log"
val input :ProvenanceRDD[TaintedString] = new FlowDebugContext(sc).textFileWithTaint(log)  

val split  = input.flatMap{s: TaintedString => 
   val tokens = s.split(",") 
   // finds the state for a zipcode
   var state = zipToState(tokens(0))
   var date = tokens(1)
   // gets snow value and converts it into millimeter
   val snow = convertToMm(tokens(2)) 
   //gets year
   val year = date.substring(date.lastIndexOf("/")) 
   // gets month / date	
   val monthdate= date.substring(0,date.lastIndexOf("/")) 
 	 List[((TaintedString,TaintedString),TaintedFloat)](
			((state , monthdate) , snow) , 
			((state , year)  , snow)
		)
}
//Delta between min and max snowfall per key group
val deltaSnow = split
 .groupByKey()
 .mapValues{ s: List[TaintedFloat]  => 
   s.max - s.min
}
deltaSnow.saveAsTextFile("hdfs://s3-92:9010/")
def convertToMm(s: TaintedString): TaintedFloat = {
  val unit = s.substring(s.length - 2)
  val v = s.substring(0, s.length - 2).toFloat
  unit match {
   case "mm" => return v
   case _ => return v * 304.8f
   }
}
\end{lstlisting}
\vspace{-2ex}
\caption{Example 1 with \tool enabled}
\label{code_example_a_bar}
\end{subfigure}
    \begin{tikzpicture}[overlay]
        % \draw[red,thick,rounded corners] (8.7,10) rectangle (16.5,11);
    %    \draw[red,thick,rounded corners] (0.3,3.97) rectangle (8,5.7);
    % \draw[red,thick,rounded corners] (0.5,0.5) rectangle (2,2);
    % jason: for some reason the reference point changed to top right, so re-edit accordingly
    \draw[red,thick,rounded corners] (-0.6,-0.55) rectangle (-8.5,-1.2);
    \end{tikzpicture}
\vspace{-2ex}
\caption{Example 1 identifies, for each state in the US, the delta between the minimum and the maximum snowfall reading for each day of any year and for any particular year. Measurements can be either in millimeters or in feet. The conversion function is described at line 27. The red rectangle highlights code edits to enable \tool's UDF-aware taint propagation. Although Scala does not require explicit types to be declared, some variable types are mentioned in orange color to highlight type difference.}

\label{code:example_a}
\end{figure*}


==> code/code_example_b.tex <==
%%%%%%%%%%%%%%%%%%%%% Example Code Figure%%%
\begin{figure}[t]
 \begin{lstlisting}
val log = "s3n://xcr:wJY@ws/logs/weather.log" 
val input :ProvenanceRDD[TaintedString]] = new FlowDebugContext(sc).textFileWithTaint(log)  

val split = input.flatMap{s: TaintedString => 
    . . . 
    }
val deltaSnow = split
 .aggregateByKey((0.0, 0.0, 0)){
   {case ((sum, sum_Sq, count), next) => 
     (sum + next, sum_sq + next * next,
                                count + 1) },
   {case ((sum1, sum_sq1, count1), 
                (sum2, sum_sq2, count2)) => 
     (sum1 + sum2, sum_sq1 + sum_sq2,
                        count1 + count2) },
    // Optional argument to enable taint propagation
    enableTaintPropagation = Some(false),
    // Optional influence function  
    influenceTrackerCtr = Some(
        () => StreamingOutlierInfluenceTracker(
                zscoreThreshold=0.96)
     )
 }.mapValues{ 
   case (sum, sum2, count) => 
     ((count*sum2) - (sum*sum))/(count*(count-1))}
    
deltaSnow.saveAsTextFile("hdfs://s3-92:9010/")
\end{lstlisting}
    \begin{tikzpicture}[overlay]
        \draw[red,thick,rounded corners] (-4,2.1) rectangle (4,6.35);
    \end{tikzpicture}
    \vspace{-4ex}
\caption{Running example 2 identifies, for each state in the US, the variance of snowfall reading for each day of any year and for any particular year. Red rectangle highlights the changes to enable influence-based provenance. }
\label{code_example_b_bar}
\vspace{-5ex}
\end{figure}

==> code/code_example_driver_collatz.tex <==
\begin{lstlisting}[language=Scala]
// Collatz program output RDD and UDF RDD
val programOutput: HybridRDD[(Int, Int), (Int, Int)] = sum 
val targetUDF: HybridRDD[(Int, Iterable[Int]), (Int, Int)] = solved

// Initial seed input dataset.
val seed = 
  Array(Array("1"), Array("2"), Array("3"), Array("4"))

// Monitor template to define the symptom: ratio of the two largest partition runtimes >= 5
val monitorTemplate: MonitorTemplate = 
  MonitorTemplate.nextComparisonThresholdMetricTemplate(
    Metrics.Runtime, thresholdFactor = 5.0)

// Map of (mutation operators -> weight) for target UDF and
// program input, built from monitor template definition and
// input data types. PerfGen can auto-generate these, but 
// users can also customize them by adjusting weights or 
// removing incompatible mutations.
val inputMutationMap: MutationMap[String] = 
  MutationMaps.buildBaseMap[String](monitorTemplate)
val udfMutationMap: MutationMap[(Int, Iterable[Int])] = 
  MutationMaps.buildTupleMapWithIterableValue[Int, Int](monitorTemplate)

val config = PerfGenConfig(
    programOutput, // HybridRDD output of entire program
    targetUDF, // HybridRDD output of target UDF
    monitorTemplate, // Monitor Template / Symptom definition
    inputMutationMap, // Program mutations
    udfMutationMap, // UDF mutations
    seed, // initial seed input
    inverse // pseudo-inverse function from Collatz program.
)

PerfGen.run(config)
\end{lstlisting}

==> code/code_fuzz_fn_outline.tex <==
\begin{lstlisting}[language=Scala]
def fuzz[T,U](progFn: RDD[T] => RDD[U], seed: RDD[T], monitor: MonitorTemplate, mutations: MutationMap[T]) = {
	val seeds = List(seed)
	var maxScore = 0.0
	while(true) { // not timed out
		// select a seed and apply a randomly selected mutation
		val base = sample(seeds)
		val newInput = mutations.sample().apply(base)
		
		val programOutput = progFn(newInput) // test the new input

		// Use monitor template to check if symptom was reproduced
		// or if feedback score was increased.
		val metrics = config.metric.getLastExecutionMetrics()
		val (meetsCriteria, feedbackScore) = monitorTemplate.checkSymptoms(metrics)
		if(meetsCriteria) { // symptom reproduced
			return newInput
		} else if (feedbackScore > maxScore) { // score increased
			maxScore = feedbackScore
			seed.append(newInput)
		}
	}
}
\end{lstlisting}

==> code/code_hybridrdd_simplified.tex <==
\begin{lstlisting}[language=Scala]
class HybridRDD[I, T](val parent: HybridRDD[_, I],
                            val computeFn: RDD[I] => RDD[T]){
    val _rdd: RDD[T] = computeFn(parent._rdd)

    // RDD-equivalent APIs that wrap Spark RDDs and 
    // decouple transformations (functions) from
    // input datasets (parents).
    def map[U](f: T=>U): HybridRDD[T, U] = 
        new HybridRDD(this, _rdd => _rdd.map(f))
    def filter(f: T > Boolean): HybridRDD[T, U] = 
        new HybridRDD(this, _rdd => _rdd.filter(f))
    ...
    def collect(): Array[T] =
        _rdd.collect()
}
\end{lstlisting}

==> code/code_monitor_template_simplified.tex <==
\begin{lstlisting}[language=Scala]
trait MonitorTemplate {
  val metric: Metric

  // Detect performance symptoms and generate feedback based on the provided metric definition.
  def checkSymptoms(partitionMetrics: Array[Long]): SymptomResult

  case class SymptomResult(meetsCriteria: Boolean, feedbackScore: Double)
}
\end{lstlisting}

==> code/code_monitor_template_threshold_example.tex <==
\begin{lstlisting}[language=Scala]
class MaximumThreshold(val threshold: Double, override val metric: Metric) extends MonitorTemplate {
  override def checkSymptoms(partitionMetrics: Array[Long]): SymptomResult = {
    val max = partitionMetrics.max
    val meetsCriteria = max >= threshold
    val feedbackScore = max
    
    return SymptomResults(meetsCriteria, feedbackScore)
  }
}
\end{lstlisting}

==> code/code_phased_fuzzing_outline.tex <==
\begin{lstlisting}[language=Scala]
def phasedFuzzing[I, U, O](conf: PerfGenConfig[I, U, O]): RDD[I] = {
// Step 1: Fuzz the target UDF to produce symptom-triggering intermediate inputs
	// partially run program up until UDF
	val udfSeed: RDD[U] = computeUDFInput(conf.seed) 
	val udfSymptomInput: RDD[U] = fuzz(conf.udfProgram,
	  udfSeed, conf.monitorTemplate, conf.udfMutations)

// Step 2: Use pseudo-inverse function to generate program seed
	val programSeed: RDD[I] = conf.inverseFn.apply(udfSymptomInput)

// Step 3: Fuzz the full program to produce symptom-triggering program inputs
	val programSymptomInput: RDD[I] = fuzz(conf.fullProgram, 
      programSeed, conf.monitorTemplate, conf.programMutations)

	return programSymptomInput
}
\end{lstlisting}

==> code/code_stockbuysell_program.tex <==
% \lstset{language=C++}
% Use mathescape to support the exclamation mark
% \begin{lstlisting}[style=MyJavaSmallStyle,mathescape=true]
\begin{lstlisting}[language=Scala,mathescape=true]
val accum = sc.collectionAccumulator("partitionCount")

val lines = HybridRDD(sc.textFile("stocks"))
val parsed = lines.map(line => {
  val split = line.split(",")
  (split(0), split(1), split(4).toDouble) })

val grouped = parsed.groupByKey()
val sortedPrices = grouped.mapValues(group => {
  val sortedDedup = SortedMap(group.toSeq: _*)
  sortedDedup.values })

val maxProfits = sortedPrices.mapPartitions(iter => {
  var partitionCounter = 0
  val dataIter: Iterator[(String, Double)] = iter.map(
    // The buy+sell algorithm
    { case (key, pricesIterable) =>
      var maxProfit = 0.0
      val prices = pricesIterable.toArray
      val memo = Array.fill(3+1)(Array.fill(prices.length)(0.0))
        
      (1 to 3).foreach(k => {
        var tmpMax = memo(k - 1)(0) - prices(0)
        (1 until prices.length).foreach(i => {
          memo(k)(i) = Math.max(memo(k)(i-1), tmpMax + prices(i))
          tmpMax = Math.max(tmpMax, memo(k-1)(i) - prices(i))
          if(memo(k)(i) > maxProfit) {
            partitionCounter += 1
            maxProfit = memo(k)(i)
          } }) })
      (key, maxProfit)
    })
    
  // Wrap iterator to update the accumulator.
  val wrappedIter = new Iterator[(String, Double)] {
    override def hasNext: Boolean = {
      if($!$dataIter.hasNext) { accum.add(partitionCounter) }
      dataIter.hasNext
    }
    override def next(): (String, Double) = dataIter.next()
  }

  wrappedIter
})
\end{lstlisting}


==> plots/time-series-subplots/collatz_timeseries.tex <==
% Adapted from BigFuzz figure 4
% Collatz plot: `
%  dashed black - UDF fuzzing
%  choice: use a diff mark to indicate difference
 \addplot[thick,smooth,mark=x,dashed] plot coordinates {
        (0.0, 1.0)
        (0.6833333333333333, 40820.0)
    };
% solid black - program fuzzing
    \addplot[ultra thin,smooth,mark=* ] 
        plot coordinates {
            (1.3833333333333333, 40907.0)
    };

%     \addplot[thin,smooth, mark=x,red,dashed] plot
% coordinates {
%         (0,0)
%         (10,50)
%         (50,50)
%         (100,50)
%         (1000,50)
%     };
% red solid - baseline    
    \addplot[thin,smooth, mark=x,red]
      plot coordinates {
            (0.0, 1.0)
(2.316666666666667, 6.0)
(2.4166666666666665, 7.0)
(2.933333333333333, 13.5)
(11.533333333333333, 32.0)
(15.583333333333334, 208.0)
    };
    
% dotted ?? - target
% https://tex.stackexchange.com/questions/192618/add-a-horizontal-line-to-a-pgfplot-and-add-it-to-the-legend
\addplot[thick, dotted, blue, samples=2,domain=0:500] {100};

    %Done

==> plots/time-series-subplots/deptgpas_coursedeptGPas.tex <==
% Adapted from BigFuzz figure 4
% Stock plot: `
%  dashed black - UDF fuzzing
%  choice: use a diff mark to indicate difference
 \addplot[thick,smooth,mark=x,dashed] plot coordinates {
        (0.0, 0.0)
(0.03333333333333333, 1.16)
(0.05, 2.08)
(0.1, 4.87)
(2.066666666666667, 4.87)
(2.35, 4.87)
(2.5166666666666666, 7.32)
(2.533333333333333, 7.32)
(2.6333333333333333, 7.32)
(2.95, 7.32)
(3.1166666666666667, 7.32)
(3.183333333333333, 31.28)
(3.5166666666666666, 31.28)
(3.65, 31.28)
(3.816666666666667, 31.28)
(4.0, 31.28)
(4.083333333333333, 184.9)
(4.15, 184.9)
    };
% solid black - program fuzzing
    \addplot[ultra thin,smooth,mark=* ] 
        plot coordinates {
            (4.15, 184.9)
    };

%     \addplot[thin,smooth, mark=x,red,dashed] plot
% coordinates {
%         (0,0)
%         (10,50)
%         (50,50)
%         (100,50)
%         (1000,50)
%     };
% red solid - baseline    
    \addplot[thin,smooth, mark=x,red]
      plot coordinates {
            (0.0, 3.0)
(29.083333333333332, 4.473684210526316)
(32.35, 4.526315789473684)
(33.916666666666664, 4.578947368421052)
(35.083333333333336, 4.631578947368421)
(35.93333333333333, 4.684210526315789)
(36.36666666666667, 4.7368421052631575)
(37.13333333333333, 4.7894736842105265)
(37.266666666666666, 4.842105263157895)
(38.3, 4.894736842105263)
(45.333333333333336, 4.947368421052632)
(46.56666666666667, 5.0)
(54.18333333333333, 5.052631578947368)
(55.21666666666667, 5.105263157894737)
(64.7, 5.157894736842105)
(66.05, 5.2105263157894735)
(66.81666666666666, 5.2631578947368425)
(68.31666666666666, 5.315789473684211)
(71.28333333333333, 5.368421052631579)
(71.6, 5.421052631578948)
(74.6, 5.473684210526316)
(76.55, 5.526315789473684)
(77.83333333333333, 5.578947368421052)
(79.21666666666667, 5.631578947368421)
(84.06666666666666, 5.684210526315789)
(93.15, 5.7368421052631575)
(103.3, 5.7894736842105265)
(106.41666666666667, 5.842105263157895)
(108.63333333333334, 5.894736842105263)
(118.51666666666667, 5.947368421052632)
(132.5, 6.0)
(141.68333333333334, 6.052631578947368)
(149.5, 6.105263157894737)
(154.01666666666668, 6.157894736842105)
(175.78333333333333, 6.2105263157894735)
(178.3, 6.2631578947368425)
(180.23333333333332, 6.315789473684211)
(192.18333333333334, 6.368421052631579)
(197.21666666666667, 6.421052631578948)
(209.3, 6.473684210526316)
(212.03333333333333, 6.526315789473684)
(215.8, 6.578947368421052)
(215.95, 6.631578947368421)
(222.01666666666668, 6.684210526315789)
            (250, 6.684210526315789) % a final point to 'carry' the line to the end of evaluation time
    };
    
\addplot[thick, dotted, blue, samples=2,domain=0:500] {100.0};

    %Done

==> plots/time-series-subplots/deptgpas_coursesGPAavgs.tex <==
% Adapted from BigFuzz figure 4
% Stock plot: `
%  dashed black - UDF fuzzing
%  choice: use a diff mark to indicate difference
 \addplot[thick,smooth,mark=x,dashed] plot coordinates {
        (0.0, 0.0)
(0.03333333333333333, 0.16)
(0.05, 1.08)
(0.1, 1.08)
(2.066666666666667, 1.08)
(2.35, 13.618279569892474)
(2.5166666666666666, 41.54545454545455)
(2.533333333333333, 41.54545454545455)
(2.6333333333333333, 101.24)
(2.95, 101.24)
(3.1166666666666667, 131.88)
(3.183333333333333, 131.88)
(3.5166666666666666, 131.88)
(3.65, 201.2)
(3.816666666666667, 201.2)
(4.0, 201.2)
(4.083333333333333, 284.9)
(4.15, 285.15789473684211)
    };
% solid black - program fuzzing
    \addplot[ultra thin,smooth,mark=* ] 
        plot coordinates {
            (4.15, 285.15789473684211)
    };

%     \addplot[thin,smooth, mark=x,red,dashed] plot
% coordinates {
%         (0,0)
%         (10,50)
%         (50,50)
%         (100,50)
%         (1000,50)
%     };
% red solid - baseline    
    \addplot[thin,smooth, mark=x,red]
      plot coordinates {
            (0.0, 3.0)
(1.4, 3.3157894736842106)
(1.5333333333333334, 3.3684210526315788)
(1.5833333333333333, 3.4210526315789473)
(2.183333333333333, 3.473684210526316)
(2.25, 3.526315789473684)
(3.4833333333333334, 3.5789473684210527)
(5.433333333333334, 3.6315789473684212)
(6.55, 3.6842105263157894)
(6.85, 3.736842105263158)
(8.2, 3.789473684210526)
(8.433333333333334, 3.8421052631578947)
(9.866666666666667, 3.8947368421052633)
(11.066666666666666, 3.9473684210526314)
(11.383333333333333, 4.0)
(11.833333333333334, 4.052631578947368)
(13.416666666666666, 4.105263157894737)
(15.016666666666667, 4.157894736842105)
(16.016666666666666, 4.2105263157894735)
(17.416666666666668, 4.2631578947368425)
(17.633333333333333, 4.315789473684211)
(25.65, 4.368421052631579)
(26.783333333333335, 4.421052631578948)
(29.083333333333332, 4.473684210526316)
(32.35, 4.526315789473684)
(33.916666666666664, 4.578947368421052)
(35.083333333333336, 4.631578947368421)
(35.93333333333333, 4.684210526315789)
(36.36666666666667, 4.7368421052631575)
(37.13333333333333, 4.7894736842105265)
(37.266666666666666, 4.842105263157895)
(100, 4.842105263157895)
(130, 4.842105263157895)
(170, 4.842105263157895)
(200, 4.842105263157895)
            (250, 6.684210526315789) % a final point to 'carry' the line to the end of evaluation time
    };
    
\addplot[thick, dotted, blue, samples=2,domain=0:500] {100.0};

    %Done

==> plots/time-series-subplots/deptgpasmedian_median.tex <==
% Adapted from BigFuzz figure 4
% Stock plot: `
%  dashed black - UDF fuzzing
%  choice: use a diff mark to indicate difference
 \addplot[thick,smooth,mark=x,dashed] plot coordinates {
        (0.0, 0.0)
(0.03333333333333333, 9.26)
(0.05, 9.26)
(0.1, 9.26)
(2.066666666666667, 9.26)
(2.35, 14.87)
(2.5166666666666666, 37.02)
(2.533333333333333, 37.03)
(2.6333333333333333, 37.03)
(2.95, 37.03)
(3.183333333333333, 72.81)
(3.5166666666666666, 72.81)
(3.65, 72.81)
(3.816666666666667, 72.81)
(4.0, 72.81)
(4.083333333333333, 214.9)
(4.15, 214.9)
    };
% solid black - program fuzzing
    \addplot[ultra thin,smooth,mark=* ] 
        plot coordinates {
            (4.15, 214.9)
    };

%     \addplot[thin,smooth, mark=x,red,dashed] plot
% coordinates {
%         (0,0)
%         (10,50)
%         (50,50)
%         (100,50)
%         (1000,50)
%     };
% red solid - baseline    
    \addplot[thin,smooth, mark=x,red]
      plot coordinates {
            (0.0, 3.0)
(0.3, 3.0526315789473686)
(0.4666666666666667, 3.1052631578947367)
(0.85, 3.1578947368421053)
(0.8666666666666667, 3.210526315789474)
(1.1333333333333333, 3.263157894736842)
(1.4, 3.3157894736842106)
(1.5333333333333334, 3.3684210526315788)
(1.5833333333333333, 3.4210526315789473)
(2.183333333333333, 3.473684210526316)
(2.25, 3.526315789473684)
(3.4833333333333334, 3.5789473684210527)
(5.433333333333334, 3.6315789473684212)
(33.916666666666664, 4.578947368421052)
(35.083333333333336, 4.631578947368421)
(35.93333333333333, 4.684210526315789)
(36.36666666666667, 4.7368421052631575)
(37.13333333333333, 4.7894736842105265)
(37.266666666666666, 4.842105263157895)
(38.3, 4.894736842105263)
(45.333333333333336, 4.947368421052632)
(46.56666666666667, 5.0)
(54.18333333333333, 5.052631578947368)
(55.21666666666667, 5.105263157894737)
(64.7, 5.157894736842105)
(66.05, 5.2105263157894735)
(66.81666666666666, 5.2631578947368425)
(68.31666666666666, 5.315789473684211)
(71.28333333333333, 5.368421052631579)
(71.6, 5.421052631578948)
(74.6, 5.473684210526316)
(76.55, 5.526315789473684)
(77.83333333333333, 5.578947368421052)
(79.21666666666667, 5.631578947368421)
(84.06666666666666, 5.684210526315789)
(93.15, 5.7368421052631575)
(103.3, 5.7894736842105265)
(106.41666666666667, 5.842105263157895)
(108.63333333333334, 5.894736842105263)
(118.51666666666667, 5.947368421052632)
(132.5, 6.0)
(141.68333333333334, 6.052631578947368)
(149.5, 6.105263157894737)
(154.01666666666668, 6.157894736842105)
(175.78333333333333, 6.2105263157894735)
(178.3, 6.2631578947368425)
(222.01666666666668, 6.684210526315789)
            (250, 6.684210526315789) % a final point to 'carry' the line to the end of evaluation time
    };
    
\addplot[thick, dotted, blue, samples=2,domain=0:500] {100.0};

    %Done

==> plots/time-series-subplots/deptgpasmedian_timeseries.tex <==
% Adapted from BigFuzz figure 4
% Stock plot: `
%  dashed black - UDF fuzzing
%  choice: use a diff mark to indicate difference
 \addplot[thick,smooth,mark=x,dashed] plot coordinates {
        (0.0, 3.0)
(0.03333333333333333, 3.05)
(0.03333333333333333, 3.1)
(0.05, 3.2)
(0.1, 3.4210526315789473)
(0.13333333333333333, 4.2105263157894735)
(0.2833333333333333, 5.2105263157894735)
(0.4166666666666667, 5.421052631578948)
(0.5666666666666667, 5.631578947368421)
(0.65, 6.578947368421052)
(0.6666666666666666, 11.421052631578947)
(0.6833333333333333, 12.052631578947368)
(0.7833333333333333, 18.526315789473685)
(0.7833333333333333, 18.57894736842105)
(0.8166666666666667, 19.526315789473685)
(0.8833333333333333, 20.0)
(1.0166666666666666, 20.05263157894737)
(1.1, 20.157894736842106)
(1.1333333333333333, 20.42105263157895)
(1.2, 21.42105263157895)
(1.2, 22.57894736842105)
(1.2666666666666666, 23.105263157894736)
(1.4166666666666667, 23.157894736842106)
(1.4666666666666666, 23.210526315789473)
(1.5, 23.31578947368421)
(1.6, 23.526315789473685)
(1.65, 24.210526315789473)
(1.6666666666666667, 24.789473684210527)
(1.7833333333333334, 41.526315789473685)
(1.8166666666666667, 47.8421052631579)
(1.95, 53.1578947368421)
(2.066666666666667, 62.94736842105263)
(2.35, 63.21052631578947)
(2.5166666666666666, 68.94736842105263)
(2.533333333333333, 69.42105263157895)
(2.6333333333333333, 69.47368421052632)
(2.95, 69.52631578947368)
(3.1166666666666667, 69.6842105263158)
(3.183333333333333, 70.78947368421052)
(3.5166666666666666, 71.36842105263158)
(3.65, 72.36842105263158)
(3.816666666666667, 84.3157894736842)
(4.0, 84.84210526315789)
(4.083333333333333, 84.89473684210526)
(4.15, 85.15789473684211)
(4.316666666666666, 353.2105263157895)
    };
% solid black - program fuzzing
    \addplot[ultra thin,smooth,mark=* ] 
        plot coordinates {
            (4.35, 353.2105263157895)
    };

%     \addplot[thin,smooth, mark=x,red,dashed] plot
% coordinates {
%         (0,0)
%         (10,50)
%         (50,50)
%         (100,50)
%         (1000,50)
%     };
% red solid - baseline    
    \addplot[thin,smooth, mark=x,red]
      plot coordinates {
            (0.0, 3.0)
(0.3, 3.0526315789473686)
(0.4666666666666667, 3.1052631578947367)
(0.85, 3.1578947368421053)
(0.8666666666666667, 3.210526315789474)
(1.1333333333333333, 3.263157894736842)
(1.4, 3.3157894736842106)
(1.5333333333333334, 3.3684210526315788)
(1.5833333333333333, 3.4210526315789473)
(2.183333333333333, 3.473684210526316)
(2.25, 3.526315789473684)
(3.4833333333333334, 3.5789473684210527)
(5.433333333333334, 3.6315789473684212)
(6.55, 3.6842105263157894)
(6.85, 3.736842105263158)
(8.2, 3.789473684210526)
(8.433333333333334, 3.8421052631578947)
(9.866666666666667, 3.8947368421052633)
(11.066666666666666, 3.9473684210526314)
(11.383333333333333, 4.0)
(11.833333333333334, 4.052631578947368)
(13.416666666666666, 4.105263157894737)
(15.016666666666667, 4.157894736842105)
(16.016666666666666, 4.2105263157894735)
(17.416666666666668, 4.2631578947368425)
(17.633333333333333, 4.315789473684211)
(25.65, 4.368421052631579)
(26.783333333333335, 4.421052631578948)
(29.083333333333332, 4.473684210526316)
(32.35, 4.526315789473684)
(33.916666666666664, 4.578947368421052)
(35.083333333333336, 4.631578947368421)
(35.93333333333333, 4.684210526315789)
(36.36666666666667, 4.7368421052631575)
(37.13333333333333, 4.7894736842105265)
(37.266666666666666, 4.842105263157895)
(38.3, 4.894736842105263)
(45.333333333333336, 4.947368421052632)
(46.56666666666667, 5.0)
(54.18333333333333, 5.052631578947368)
(55.21666666666667, 5.105263157894737)
(64.7, 5.157894736842105)
(66.05, 5.2105263157894735)
(66.81666666666666, 5.2631578947368425)
(68.31666666666666, 5.315789473684211)
(71.28333333333333, 5.368421052631579)
(71.6, 5.421052631578948)
(74.6, 5.473684210526316)
(76.55, 5.526315789473684)
(77.83333333333333, 5.578947368421052)
(79.21666666666667, 5.631578947368421)
(84.06666666666666, 5.684210526315789)
(93.15, 5.7368421052631575)
(103.3, 5.7894736842105265)
(106.41666666666667, 5.842105263157895)
(108.63333333333334, 5.894736842105263)
(118.51666666666667, 5.947368421052632)
(132.5, 6.0)
(141.68333333333334, 6.052631578947368)
(149.5, 6.105263157894737)
(154.01666666666668, 6.157894736842105)
(175.78333333333333, 6.2105263157894735)
(178.3, 6.2631578947368425)
(180.23333333333332, 6.315789473684211)
(192.18333333333334, 6.368421052631579)
(197.21666666666667, 6.421052631578948)
(209.3, 6.473684210526316)
(212.03333333333333, 6.526315789473684)
(215.8, 6.578947368421052)
(215.95, 6.631578947368421)
(222.01666666666668, 6.684210526315789)
            (250, 6.684210526315789) % a final point to 'carry' the line to the end of evaluation time
    };
    
\addplot[thick, dotted, blue, samples=2,domain=0:500] {100.0};

    %Done

==> plots/time-series-subplots/stockbuysell_timeseries.tex <==
% Adapted from BigFuzz figure 4
% Stock plot: `
%  dashed black - UDF fuzzing
%  choice: use a diff mark to indicate difference
 \addplot[thick,smooth,mark=x,dashed] plot coordinates {
        (0,1.853211009)
        (0.03333333333,2.04587156)
        (0.08333333333,2.110091743)
        (0.1166666667,2.12962963)
        (0.15,2.388888889)
        (0.15,2.574074074)
        (0.1666666667,2.583333333)
        (0.1833333333,2.622641509)
        (0.1833333333,2.635514019)
        (0.2166666667,2.722222222)
        (0.25,2.989247312)
        (0.2666666667,3.065217391)
        (0.3666666667,3.239130435)
        (0.45,3.30952381)
        (0.4833333333,3.547619048)
        (0.6,3.595238095)
        (0.6166666667,3.928571429)
        (0.8666666667,4.520547945)
        (1.116666667,4.647887324)
        (2.8,4.714285714)
        (2.866666667,4.782608696)
        (3.016666667,4.852941176)
        (3.416666667,5.076923077)
    };
% solid black - program fuzzing
    \addplot[ultra thin,smooth,mark=* ] 
        plot coordinates {
            (3.433333333,5.076923077)
    };

%     \addplot[thin,smooth, mark=x,red,dashed] plot
% coordinates {
%         (0,0)
%         (10,50)
%         (50,50)
%         (100,50)
%         (1000,50)
%     };
% red solid - baseline    
    \addplot[thin,smooth, mark=x,red]
      plot coordinates {
            (0,1.853211009)
            (0.03333333333,1.87037037)
            (0.05,1.87962963)
            (0.2666666667,1.888888889)
            (0.7833333333,1.898148148)
            (2.033333333,1.935185185)
            (2.516666667,1.962962963)
            (2.716666667,1.981481481)
            (3,2.037037037)
            (8.9,2.055555556)
            (9.316666667,2.092592593)
            (21.3,2.101851852)
            (26.53333333,2.157407407)
            (27.18333333,2.175925926)
            (32.03333333,2.185185185)
            (36.9,2.212962963)
            (43.38333333,2.268518519)
            (44.3,2.277777778)
            (45.01666667,2.324074074)
            (57.01666667,2.351851852)
            (60.96666667,2.361111111)
            (70.18333333,2.37037037)
            (74.38333333,2.407407407)
            (82.88333333,2.425925926)
            (96.05,2.444444444)
            (106.75,2.472222222)
            (115.3,2.481481481)
            (140.9333333,2.509259259)
            (189.4666667,2.518518519)
            (250,2.518518519) % a final point to 'carry' the line to the end of evaluation time
    };
    
% dotted ?? - target
% https://tex.stackexchange.com/questions/192618/add-a-horizontal-line-to-a-pgfplot-and-add-it-to-the-legend
\addplot[thick, dotted, blue, samples=2,domain=0:500] {5.0};

    %Done

==> plots/time-series-subplots/stockbuysell_timeseries_orig.tex <==
% Adapted from BigFuzz figure 4
% Stock plot: `
%  dashed black - UDF fuzzing
%  choice: use a diff mark to indicate difference
 \addplot[ultra thin,smooth,mark=x,dashed] plot coordinates {
        (0,1.853211009)
        (0.03333333333,2.04587156)
        (0.08333333333,2.110091743)
        (0.1166666667,2.12962963)
        (0.15,2.388888889)
        (0.15,2.574074074)
        (0.1666666667,2.583333333)
        (0.1833333333,2.622641509)
        (0.1833333333,2.635514019)
        (0.2166666667,2.722222222)
        (0.25,2.989247312)
        (0.2666666667,3.065217391)
        (0.3666666667,3.239130435)
        (0.45,3.30952381)
        (0.4833333333,3.547619048)
        (0.6,3.595238095)
        (0.6166666667,3.928571429)
        (0.8666666667,4.520547945)
        (1.116666667,4.647887324)
        (2.8,4.714285714)
        (2.866666667,4.782608696)
        (3.016666667,4.852941176)
        (3.416666667,5.076923077)
    };
% solid black - program fuzzing
    \addplot[ultra thin,smooth,mark=* ] 
        plot coordinates {
            (3.433333333,5.076923077)
    };

%     \addplot[thin,smooth, mark=x,red,dashed] plot
% coordinates {
%         (0,0)
%         (10,50)
%         (50,50)
%         (100,50)
%         (1000,50)
%     };
% red solid - baseline    
    \addplot[thin,smooth, mark=*,red]
      plot coordinates {
            (0,1.853211009)
            (0.03333333333,1.87037037)
            (0.05,1.87962963)
            (0.2666666667,1.888888889)
            (0.7833333333,1.898148148)
            (2.033333333,1.935185185)
            (2.516666667,1.962962963)
            (2.716666667,1.981481481)
            (3,2.037037037)
            (8.9,2.055555556)
            (9.316666667,2.092592593)
            (21.3,2.101851852)
            (26.53333333,2.157407407)
            (27.18333333,2.175925926)
            (32.03333333,2.185185185)
            (36.9,2.212962963)
            (43.38333333,2.268518519)
            (44.3,2.277777778)
            (45.01666667,2.324074074)
            (57.01666667,2.351851852)
            (60.96666667,2.361111111)
            (70.18333333,2.37037037)
            (74.38333333,2.407407407)
            (82.88333333,2.425925926)
            (96.05,2.444444444)
            (106.75,2.472222222)
            (115.3,2.481481481)
            (140.9333333,2.509259259)
            (189.4666667,2.518518519)
            (250,2.518518519) % a final point to 'carry' the line to the end of evaluation time
    };
    
% dotted ?? - target
% https://tex.stackexchange.com/questions/192618/add-a-horizontal-line-to-a-pgfplot-and-add-it-to-the-legend
\addplot[thick, dotted, blue, samples=2,domain=0:500] {5.0};

    %Done

==> plots/time-series-subplots/wordcount_timeseries.tex <==
% Adapted from BigFuzz figure 4
% Stock plot: `
%  dashed black - UDF fuzzing
%  choice: use a diff mark to indicate difference
 \addplot[thick,smooth,mark=x,dashed] plot coordinates {
        (0.0, 0.32597954540411533)
(0.1, 0.3478877915544592)
(0.18333333333333332, 0.3503034215025946)
(0.35, 0.7002454868190077)
(0.5, 0.7019188375525316)
(0.65, 0.8797697758951392)
(0.7833333333333333, 0.8799395542707441)
(0.8833333333333333, 1.1694142029402117)
(1.1833333333333333, 1.2797986962488233)
(1.2833333333333334, 1.279798696248824)
(1.3833333333333333, 1.351641922113788)
(1.45, 1.388488234822856)
(1.5, 1.3884882348228567)
(2.3666666666666667, 1.47727527043603)
(2.55, 1.5211967228671355)
(2.566666666666667, 1.5211967228671357)
(4.1, 1.8934854137220265)
(4.583333333333333, 1.8943624697154682)
(5.45, 1.9811344212271025)
(6.266666666666667, 2.1309312900796167)
    };
% solid black - program fuzzing
    \addplot[ultra thin,smooth,mark=* ] 
        plot coordinates {
            (6.3, 2.131650642174522)
    };

%     \addplot[thin,smooth, mark=x,red,dashed] plot
% coordinates {
%         (0,0)
%         (10,50)
%         (50,50)
%         (100,50)
%         (1000,50)
%     };
% red solid - baseline    
    \addplot[thin,smooth, mark=x,red]
      plot coordinates {
            (0.0, 0.32597954540411517)
(0.03333333333333333, 0.3260272132501107)
(0.06666666666666667, 0.32760172588015835)
(0.13333333333333333, 0.3277052403182269)
(0.15, 0.3289963902070682)
(0.18333333333333332, 0.3295287333909111)
(0.2, 0.3305571309843411)
(0.2, 0.33142991070825123)
(0.23333333333333334, 0.3324156557289627)
(0.4166666666666667, 0.3338310614362525)
(0.55, 0.3342263091030877)
(0.5833333333333334, 0.3342828581797626)
(0.6833333333333333, 0.3347071332765725)
(0.7166666666666667, 0.33630431607627553)
(0.9, 0.33728875774889233)
(0.9166666666666666, 0.33773150743697017)
(0.95, 0.33773150743697034)
(1.0166666666666666, 0.3381597452106927)
(1.4833333333333334, 0.3393148133305977)
(1.6166666666666667, 0.34017868456006994)
(1.7833333333333334, 0.3406103583251101)
(2.1166666666666667, 0.3424314226082026)
(2.25, 0.3430781290659952)
(2.316666666666667, 0.34598703757307286)
(2.933333333333333, 0.34738478817017143)
(3.066666666666667, 0.34921194612684847)
(3.433333333333333, 0.3506209842943156)
(3.5, 0.3535201212859308)
(3.9, 0.3553337700613013)
(4.45, 0.35540939988281944)
(4.65, 0.3563201517381821)
(4.916666666666667, 0.3563979255133062)
(5.016666666666667, 0.36002422796974)
(5.05, 0.3629405540607429)
(5.083333333333333, 0.3658661980656376)
(6.6, 0.3688011060226029)
(7.5, 0.3696999711387116)
(7.6, 0.3717452239186117)
(7.633333333333334, 0.3735606559587651)
(7.666666666666667, 0.375185012714108)
(7.683333333333334, 0.3783090854980853)
(9.216666666666667, 0.3868559377692802)
(9.366666666666667, 0.3899035322637399)
(10.416666666666666, 0.3918031835259219)
(11.116666666666667, 0.3928436682144002)
(11.55, 0.39368902522421684)
(11.6, 0.39486047603183094)
(12.15, 0.39674685853413316)
(12.533333333333333, 0.39861941698933934)
(13.3, 0.3987223003373389)
(14.333333333333334, 0.3996716507197421)
(14.45, 0.4011559075450014)
(14.883333333333333, 0.40115590754500163)
(14.983333333333333, 0.4016869223705712)
(15.066666666666666, 0.4042139222435599)
(15.65, 0.40432163807446386)
(16.233333333333334, 0.4072810117251748)
(16.4, 0.40728101172517484)
(16.433333333333334, 0.408981757214563)
(16.533333333333335, 0.4108526544591801)
(16.716666666666665, 0.4123262087386731)
(17.933333333333334, 0.41296946106722016)
(18.483333333333334, 0.41483128807711606)
(18.65, 0.4158760771792094)
(18.783333333333335, 0.41772920653087775)
(18.833333333333332, 0.41772920653087803)
(19.916666666666668, 0.4207962570371105)
(20.783333333333335, 0.4238722677994937)
(22.383333333333333, 0.42531650442266045)
(22.65, 0.4253165044226605)
(23.133333333333333, 0.42635526479770564)
(23.333333333333332, 0.4273803495277355)
(24.016666666666666, 0.4278115508265726)
(24.05, 0.42793624437984756)
(24.7, 0.4308762335595782)
(25.133333333333333, 0.43233375327733925)
(25.516666666666666, 0.43336016355918877)
(26.0, 0.4334895923324911)
(26.766666666666666, 0.4351988063472779)
(26.95, 0.43618393902340236)
(27.933333333333334, 0.43788398781705345)
(28.083333333333332, 0.43804739290671263)
(28.366666666666667, 0.4395163973453254)
(28.633333333333333, 0.4409523561322048)
(28.65, 0.44107979837190314)
(28.816666666666666, 0.4440295572782769)
(30.133333333333333, 0.4459005152362532)
(31.4, 0.4471155338907862)
(31.716666666666665, 0.4489869993350091)
(32.266666666666666, 0.44898699933500913)
(33.68333333333333, 0.45084458438728686)
(34.43333333333333, 0.4600452981125283)
(35.333333333333336, 0.46437663178609445)
(37.55, 0.4653786997478806)
(38.083333333333336, 0.46609478261308407)
(38.36666666666667, 0.46624063462139936)
(38.45, 0.4684898988039935)
(38.65, 0.46954954861031334)
(39.36666666666667, 0.4705953841732748)
(40.06666666666667, 0.4720250853274351)
(40.083333333333336, 0.47625211685659574)
(40.5, 0.47639070903318004)
(40.9, 0.479381438343757)
(41.3, 0.48040218511499194)
(41.71666666666667, 0.48040218511499205)
(42.083333333333336, 0.48183976372305204)
(42.55, 0.48328932584290135)
(43.166666666666664, 0.4864063127827457)
(44.166666666666664, 0.4895318458924714)
(45.2, 0.49125913263179677)
(48.9, 0.4929723009728153)
(49.78333333333333, 0.49441027326782977)
(50.3, 0.4961075818659348)
(51.1, 0.4971984738386981)
(52.13333333333333, 0.4973558851696366)
(52.7, 0.49780725986712127)
(52.7, 0.49862526250376343)
(53.266666666666666, 0.49923346392032997)
(53.71666666666667, 0.5009516240613199)
(54.016666666666666, 0.5026378182243142)
(54.13333333333333, 0.5026378182243143)
(55.733333333333334, 0.5057912229796768)
(56.36666666666667, 0.508952948521158)
(58.21666666666667, 0.5091191089642813)
(59.03333333333333, 0.5122908373510274)
(65.58333333333333, 0.5136726632227299)
(67.51666666666667, 0.5153489544581326)
(69.13333333333334, 0.5167419603241884)
(69.26666666666667, 0.5178541962707629)
(69.91666666666667, 0.5195205109361702)
(71.4, 0.52117267613553)
(71.63333333333334, 0.5213407985100983)
(73.7, 0.5222272563829051)
(74.03333333333333, 0.5253893881263969)
(75.05, 0.5285597017808569)
(76.26666666666667, 0.5302037438636866)
(80.2, 0.5313225843829875)
(81.83333333333333, 0.5332860876451968)
(82.81666666666666, 0.5333828679198369)
(82.98333333333333, 0.5334683710419004)
(84.46666666666667, 0.5347521002237475)
(84.73333333333333, 0.5358719090602974)
(84.95, 0.537834774895768)
(86.35, 0.5410123541365117)
(90.7, 0.5410123541365119)
(90.73333333333333, 0.5441979591342943)
(91.53333333333333, 0.5453113554402166)
(92.9, 0.5466687599002777)
(94.85, 0.5477680425637106)
(94.93333333333334, 0.5491370596782571)
(96.16666666666667, 0.5494191717432227)
(97.41666666666667, 0.5502222603262381)
(98.06666666666666, 0.5504184814245827)
(98.38333333333334, 0.5526045588179149)
(99.41666666666667, 0.5526847155391176)
(99.63333333333334, 0.5533969757831757)
(99.83333333333333, 0.5542421713703385)
(101.83333333333333, 0.5544694142163457)
(102.55, 0.5553202949044013)
(102.9, 0.5555234224671624)
(103.18333333333334, 0.5555456165382714)
(103.43333333333334, 0.5557978734172718)
(103.78333333333333, 0.5572107493182483)
(103.81666666666666, 0.5572974171059176)
(103.86666666666666, 0.5595670579223319)
(104.33333333333333, 0.5597695084368158)
(105.43333333333334, 0.5604929037315494)
(106.35, 0.561748198152051)
(106.83333333333333, 0.5621279565900192)
(108.0, 0.5637127364859772)
(109.58333333333333, 0.5669035852220158)
(110.0, 0.5679803970543778)
(111.23333333333333, 0.5693193142063)
(111.6, 0.5695205522307004)
(112.33333333333333, 0.5709659980269666)
(112.51666666666667, 0.5720868065372641)
(114.43333333333334, 0.5741553253691368)
(115.01666666666667, 0.5761167230065279)
(116.75, 0.5773524815503845)
(116.93333333333334, 0.5774544064969969)
(117.03333333333333, 0.5789862107686448)
(118.08333333333333, 0.5806056896879338)
(118.81666666666666, 0.580954197627525)
(119.18333333333334, 0.5811677932264948)
(119.4, 0.5824940665553093)
(122.53333333333333, 0.5825799166381239)
(122.65, 0.5898904248990655)
(138.11666666666667, 0.5918575030657605)
(139.21666666666667, 0.5920528665856806)
(140.3, 0.5937198021694023)
(141.66666666666666, 0.5948031489557685)
(143.76666666666668, 0.5950343965187233)
(145.46666666666667, 0.5967705421524718)
(145.78333333333333, 0.5978448957713557)
(147.65, 0.599513068162119)
(147.91666666666666, 0.5999510603496863)
(149.11666666666667, 0.6001441424295566)
(149.25, 0.6012939031936876)
(149.88333333333333, 0.6026952678587922)
(150.16666666666666, 0.6040190490826128)
(152.4, 0.6056726063964829)
(152.86666666666667, 0.6076425050514488)
(153.85, 0.6076425050514489)
(157.13333333333333, 0.6108220721335794)
(158.41666666666666, 0.6124680548151147)
(163.11666666666667, 0.6126774147138002)
(163.26666666666668, 0.6140093969011124)
(163.55, 0.6159654855604778)
(166.81666666666666, 0.6179072112679281)
(170.41666666666666, 0.6195662049960228)
(177.03333333333333, 0.6208742200838507)
(177.11666666666667, 0.6211028042994069)
(177.7, 0.6230304455006365)
(187.03333333333333, 0.6249436874233094)
(188.98333333333332, 0.6261334343570806)
(189.46666666666667, 0.6293382866850581)
(199.46666666666667, 0.6310155881669595)
(201.21666666666667, 0.63101558816696)
(205.91666666666666, 0.6322984047150001)
(206.38333333333333, 0.6329260863692556)
(206.83333333333334, 0.6339603800323348)
(207.3, 0.6352540997700278)
(209.73333333333332, 0.6369007660738638)
(216.66666666666666, 0.6400922389347129)
(221.11666666666667, 0.6400922389347132)
(225.68333333333334, 0.6413855141810886)
(226.53333333333333, 0.6445732210304641)
(226.61666666666667, 0.6448131297989208)
(227.25, 0.6462057123944998)
(227.28333333333333, 0.6464931844893161)
(228.23333333333332, 0.6481317418232511)
(232.11666666666667, 0.6513277994556167)
(235.48333333333332, 0.6545313267830062)
(236.13333333333333, 0.6561565303197442)
(239.23333333333332, 0.6577672604289719)
(250, 0.6577672604289719) % a final point to 'carry' the line to the end of evaluation time
    };
    
% dotted ?? - target
% https://tex.stackexchange.com/questions/192618/add-a-horizontal-line-to-a-pgfplot-and-add-it-to-the-legend
\addplot[thick, dotted, blue, samples=2,domain=0:500] {2.0};

    %Done

==> tables/collatz_mutations_weights.tex <==
\begin{tabular}{|c|c|c|}
\cellcolor{black}{\textcolor{white}{\at{\bf Mutation~Operators}}}
& \cellcolor{black}{\textcolor{white}{\at{\bf Weight}}}
& \cellcolor{black}{\textcolor{white}{\at{\bf Sampling~\%}}}
\\\hline
M10 + M7 + M1 & 1.0 & 11.1\%
\\\hline
M10 + M7 + M1 + M5 & 5.0 & 55.5\%
\\\hline
M10 + M7 + M6 & 1.0 & 11.1\%
\\\hline
M11 & 0.5 & 5.6\%
\\\hline
M12 & 0.5 & 5.6\%
\\\hline
M14 & 1.0 & 11.1\%
\\\hline
\end{tabular}

==> tables/collatz_results.tex <==
\begin{tabular}{| c || r | r |}
\cellcolor{black}{\textcolor{white}{\at{\bf Fuzzing\ Step}}}
& \cellcolor{black}{\textcolor{white}{\at{\bf Duration\ (ms)}}}
&\cellcolor{black}{\textcolor{white}{\at{\bf \#Iterations}}}
\\\hline
\hspace{-1ex}
UDF Fuzzing (\perfgen) & 30385	& 34
\\\hline
\makecell{Program Fuzzing with\\ Improved Seed (\perfgen)} & 27180 & 1
\\\hline
Phased Fuzzing (\perfgen) & 57702 & 1
\\\hline
\makecell{Program Fuzzing with\\ Original Seed (Baseline)} & 2668253 &	58426
\\\hline
\end{tabular}

==> tables/deptgpamedian_results.tex <==
% New format that includes additional rows for seed generation...
% /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220224/deptgpaquartile_recread/nextcmp_1000_dupe50_baseline/
% /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220315/deptgpaquartiles_nxtcmp100_dupe5/
\begin{tabular}{| c || r | r |}
\cellcolor{black}{\textcolor{white}{\at{\bf Fuzzing\ Step}}}
& \cellcolor{black}{\textcolor{white}{\at{\bf Duration\ (ms)}}}
&\cellcolor{black}{\textcolor{white}{\at{\bf \#Iterations}}}
\\\hline
\hspace{-1ex}
Intermediate Seed Computation & 2282 & -
\\\hline
UDF Fuzzing & 259205 & 1519
\\\hline
Inverse Function Application & 736 & -
\\\hline
\makecell{End-to-end Fuzzing with\\ Improved Seed (\perfgen)} & 638 & 1
\\\hline
\perfgen Total & 262864 & -
\\\hline
Baseline & 14403113 & 21575*
\\\hline
\end{tabular}

==> tables/evaluation_results.tex <==
%% Table for influence functions, 
\begin{tabular}{| c | r | r | c | r | r | r | r | r | r | r | r | r |}

 \cellcolor{black}{\textcolor{white}{\at{Subject}}}
 &  \multicolumn{1}{|c|}{\cellcolor{black}{\textcolor{white}{\at{Input}}}}
 & \multicolumn{1}{|c|}{\cellcolor{black}{\textcolor{white}{\at{Faulty}}}}
& \cellcolor{black}{\textcolor{white}{\at{\perfgen}}}
& \multicolumn{3}{c}{\cellcolor{black}{\textcolor{white}{\at{Trace\ Size}}}} & \multicolumn{3}{c}{\cellcolor{black}{\textcolor{white}{\at{Precision~\%}}}} & \multicolumn{3}{c}{\cellcolor{black}{\textcolor{white}{\at{Recall~\%}}}}\\
 \cellcolor{black}{\textcolor{white}{\at{Program}}} &\cellcolor{black}{\textcolor{white}{\at{Records}}} &\cellcolor{black}{\textcolor{white}{\at{Outputs}}} &\cellcolor{black}{\textcolor{white}{\at{Strategy}}} &\cellcolor{black}{\textcolor{white}{\at{\titian}}} &\cellcolor{black}{\textcolor{white}{\at{\bigsift}}} &\cellcolor{black}{\textcolor{white}{\at{\perfgen}}} &\cellcolor{black}{\textcolor{white}{\at{\titian}}} &\cellcolor{black}{\textcolor{white}{\at{\bigsift}}} &\cellcolor{black}{\textcolor{white}{\at{\perfgen}}} &\cellcolor{black}{\textcolor{white}{\at{\titian}}} &\cellcolor{black}{\textcolor{white}{\at{\bigsift}}} &\cellcolor{black}{\textcolor{white}{\at{\perfgen}}}  
\\\hline
\hspace{-1ex}
Weather & 42.1M & 40 & UDF-Aware Tainting & 6,063,000 & 2 & 112 & 0.0 & 50.0 & 35.7 & 100.0 & 2.5 & 100.0
\\\hline
Airport & 36.0M & 34 & StreamingOutlier(z=3) & 773,760 & 1 & 34 & 0.0 & 100.0 & 100.0 & 100.0 & 2.9 & 100.0
\\\hline
Department GPA & 25.0M & 50,370 & StreamingOutlier(z=3)& - & - & 50,370 & - & - & 100.0 & - & - & 100.0
\\\hline
Course Avg & 50.0M & 24 & UDF-Aware Tainting, Top2+Bottom2 & - & - & 20 & - & - & 20.0 & - & - & 16.7
\\\hline
Student Info  & 25.0M & 31 & StreamingOutlier(z=3) & 6,247,562 & 1 & 31 & 0.0 & 100.0 & 100.0 & 100.0 & 3.2 & 100.0
\\\hline
Commute Type & 25.0M & 150 & TopN(N=1000) & 9,545,636 & 1 & 1000 & 0.0 & 100.0 & 15.0 & 100.0 & 0.7 & 100.0
\\\hline
\end{tabular}

==> tables/influence_functions.tex <==
%% Table for influence functions, 
\begin{tabular}{| c | l | l |}
\cellcolor{black}{\textcolor{white}{\at{Influence Function}}}
&\cellcolor{black}{\textcolor{white}{\at{Parameters}}}
&\cellcolor{black}{\textcolor{white}{\at{Description}}}
\\\hline
\hspace{-1ex}
All & None & \makecell[l]{Retain all provenance IDs. This is the default behavior used in transformation level provenance, when no \\ additional UDF information is available}.
\\\hline
TopN/BottomN & N (integer) & \makecell[l]{Retain provenance of the \textit{N} largest/smallest values.}
\\\hline
Custom Filter & FilterFn (boolean function) & \makecell[l]{Use a provided Scala boolean filter function (\textit{FilterFn}) to evaluate whether or not to retain provenance for\\ consumed values.} 
\\\hline
StreamingOutlier & Z (integer), BufferSize (integer) & \makecell[l]{Retain values that are considered outliers as defined by \textit{Z} standard deviations from the (streaming) mean,\\ evaluated after \textit{BufferSize} values are consumed. The default values are \textit{Z}=3, \textit{BufferSize}=1000.}
\\\hline
Union & \makecell[l]{InfluenceFunctions\\(1+ Influence Functions)} & \makecell[l]{Apply each provided influence function and calculate the union of provenance across all functions.}
\\\hline
\end{tabular}

==> tables/metric_templates_old.tex <==
%% Table for Metric Templates
% Discussion/Thoughts:
% Data Skew: Metrics: ratio-based is any 
% 
\begin{tabular}{| c | c | c | c| p{0.4\linewidth} |}
\cellcolor{black}{\textcolor{white}{\at{\bf Type}}}
&\cellcolor{black}{\textcolor{white}{\at{\bf Parameters}}}
&\cellcolor{black}{\textcolor{white}{\at{\bf Feedback\ Score}}}
&\cellcolor{black}{\textcolor{white}{\at{\bf Condition}}}
&\cellcolor{black}{\textcolor{white}{\at{\bf Description}}}
\\\hline
% \hspace{-1ex}
\makecell{Interquartile Range (IQR)\\ Outlier} & \makecell{IQR distance threshold \textit{t}\\(default 1.5)} & \makecell{$\max(x_{(n)} - Q3, Q1 - x_1)$ \\$/ (Q3-Q1)$} & $ score \ge t$ & Computes the differences of (1) the first quartile and smallest partition metric and (2) the third quartile and largest partition metric, normalized by the Interquartile Range (IQR). The larger of these two distances is returned as the feedback score, and the monitored program execution is determined to exhibit performance skew if this value exceeds the \textit{IQR distance threshold}, which traditionally defaults to 1.5.
\\\hline
Skewness & \makecell{upper bound \textit{u}\\ (default 1.0), \\{[lower bound \textit{l}]}} & \makecell{skewness: $m_3/s^3$\\where $m_3$ = third central moment,\\$s$ = sample standard deviation} & \makecell{$score \ge u$\\$[$or $score \le l]$} & Computes the skewness of the partition metrics distribution and checks if it falls outside the specified bounds.
\\\hline
\makecell{Partition Skew Ratio} & \makecell{Target ratio $r$,\\ {[minimum threshold $m$]}} & $x_{(n)} / avg(x_{1...(n-1)})$ & \makecell{$score \ge r \And$\\$x_{(n)} \ge m$} & Computes the ratio between each partition's metric and the average of all other partitions' metrics. If the largest such ratio is greater than \textit{target factor}, the monitored program execution is determined to exhibit performance skew. An optional \textit{minimum threshold} is used to establish a minimum metric value before a ratio is computed and is useful in filtering out situations where executions are too fast or trivial to reliably detect performance skew (\eg comparing a 3 ms partition metric vs a remaining average of 1 ms)
\\\hline
Error Detection & \makecell{Error message substring $s$, \\ underlying template $t$} & $t.score()$ & \makecell{error thrown and \\ $msg.contains(s)$} & Monitors executions for performance skew in the form of an error containing the specified \textit{error message substring}. This implementation requires an additional \textit{underlying template} which is used to guide fuzzing towards the desired error, but is not used in detecting performance skew symptoms.
\\\hline
%  \todo{order}
Maximum Threshold & value threshold $t$ & maximum metric value $x_{(n)}$ & $score \ge t$ & Computes the maximum metric value and checks if it exceeds a predefined threshold.
\\\hline
Next Comparison & ratio threshold $t$ & $x_{(n)}/x_{(n-1)}$  & $score \ge t$ & Computes the ratio between the two largest metric values and compares it to a specified threshold.
\\\hline
Z-Score & Z-score threshold $t$ & $(x_{(n)} - \mu)  / \sigma $ & $score \ge t$ & Computes the Z-score for the largest metric value and compares it against a predefined threshold. \todo{Discuss outlier focuses anywhere?}
\\\hline
Modified Z-Score & \makecell{Modified Z-score \\threshold $t$} & \makecell{$(x_{(n)} - M)  / 1.486*MAD $\\where $M$ = median,\\$MAD$ = median absolute deviation} & $score \ge t$ & Computes the Modified Z-score for the largest metric value and compares it against a predefined threshold.
\\\hline
\end{tabular}
% \footnote{https://en.wikipedia.org/wiki/Interquartile\_range}
% \footnote{https://en.wikipedia.org/wiki/Skewness} 

==> tables/mutations_pre-rename.tex <==
% \todo{Convert this to a full-pagewidth table. Columns should be Name, Definition(s), Type(s) (e.g. base type vs collection vs tuple), Target metric/skew. Optional/additional could be example and/or justification}.
% Outline: include base types of String, int, double, boolean
\begin{tabular}{| c | c | c | c | p{0.7\linewidth} |}
\cellcolor{black}{\textcolor{white}{\at{\bf ID}}}
& \cellcolor{black}{\textcolor{white}{\at{\bf Name}}}
& \cellcolor{black}{\textcolor{white}{\at{\bf Data\ Type}}}
&\cellcolor{black}{\textcolor{white}{\at{\bf Target\ Skew(s)}}}
&\cellcolor{black}{\textcolor{white}{\at{\bf Description}}}
\\\hline
\hspace{-1ex}
M1 & RandomInteger & Integer & Computation & Replace the input integer with a randomly generated integer value within a configurable range (default: [0, \codefont{Int.MaxValue})).
\\\hline
M2 & RandomDouble & Double & Computation & Replace the input double with a randomly generated double value within a configurable range (default: [0, \codefont{Double.MaxValue}))
\\\hline
M3 & RandomBoolean & Boolean & Computation & Replace the input boolean with a random boolean value.
\\\hline
M4 & ReplaceSubtring & String & Computation & Mutate a string by replacing a random substring (including either empty or the full string) with a newly generated random string of random length within a configurable range (default: [0, 25)).
\\\hline
M5 & CollectionElementMutation & Collection & Computation & Randomly select and mutate a random element within a collection according to its type.
\\\hline
M6 & CollectionConcatenation & Collection & \makecell{Computation,\\ Data, Memory} & Extend a collection by appending a copy of itself.
\\\hline
M7 & TupleElementMutation & 2-Element Tuple & Computation & Randomly select and mutate an element within a two-element tuple according to its type.
\\\hline
M8 & TripleElementMutation & 3-Element Tuple & Computation & Randomly select and mutate an element within a three-element tuple according to its type. 
\\\hline
M9 & QuadrupleElementMutation & 4-Element Tuple & Computation & Randomly select and mutate an element within a four-element tuple according to its type.
\\\hline
M10 & RandomRecord & Dataset & Computation & Randomly select a record and mutate it according to one of the mutations applicable to the dataset type. For example, this mutation could choose a random integer out of a integer dataset and apply the \textit{RandomInteger} mutation. 
\\\hline
M11 & KeyEnumeration & 2-Element Tuple Dataset & Data, Memory & Randomly select a random record. For each distinct value within that record's partition, append a new record to the partition consisting of the the selected record's key and the distinct value, such that the key is paired with every value in the partition.
\\\hline
M12 & ValueEnumeration & 2-Element Tuple Dataset & Data & Similar to \textit{KeyEnumeration} but instead pairing a random record's value with all distinct keys in a partition.
\\\hline
M13 & DuplicateKeyGeneration & 2-Element Tuple Dataset & Data, Memory & Randomly select a random record. Append additional records consisting of that record's key paired with mutations of its value some number of times (default: up to 10\% of partition size).
\\\hline
M14 & DuplicateValueGeneration & 2-Element Tuple Dataset & Data & Similar to \textit{DuplicateKeyGeneration} but instead with a fixed value and mutated keys.
\\\hline
\end{tabular}

==> tables/perf_metrics.tex <==

\begin{tabular}{| c | c | p{0.5\linewidth} |}
\cellcolor{black}{\textcolor{white}{\at{\bf Name}}}
&\cellcolor{black}{\textcolor{white}{\at{\bf Skew\ Category}}}
&\cellcolor{black}{\textcolor{white}{\at{\bf Description}}}
\\\hline
\hspace{-1ex}
Runtime & \makecell{Computation\\Data} & Time spent (ms) computing a single partition's result.
\\\hline
Garbage Collection & Memory & Time spent (ms) by the JVM running garbage collection to free up memory.
\\\hline
Peak Memory & Memory & Maximum memory usage (bytes) from all Spark-internal data structures used to handle data shuffling and aggregation.
\\\hline
Memory Bytes Spilled & Memory & Number of bytes spilled to disk from all Spark-internal data structures used to handle data shuffling and aggregation.
\\\hline
Input Read Records & Data & Number of records read from an input source (non-shuffle).
\\\hline
Output Write Records & Data & Number of records written to an output destination (non-shuffle).
\\\hline
Shuffle Read Records & Data & Number of records read from shuffle inputs.
\\\hline
Shuffle Read Bytes & Data & Number of bytes read from shuffle inputs.
\\\hline
Shuffle Write Records & Data & Number of records written to shuffle outputs.
\\\hline
Shuffle Write Bytes & Data & Number of bytes written to shuffle outputs.
\\\hline
\end{tabular}

==> tables/prose_results.tex <==
\begin{tabular}{| l | l | l | l | l | l |}
\hline
Original Input & \textbf{12} &\textbf{19} & \textbf{28}  & \textbf{26} &\textbf{27}% &\textbf{94}
\\\hline
Intermediate Output & \textbf{12,10} & \textbf{19,21} & \textbf{28,19} & \textbf{26,11}  &\textbf{27,111} % &\textbf{94,105}
\\\hline
Inverse Function & \multicolumn{5}{c |}{\texttt{\footnotesize SubString(v,AbsPos(v,1), AbsPos(v,2))}}
\\\hline

\end{tabular}

==> tables/stockbuysell_results.tex <==
% New format that includes additional rows for seed generation...
% /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220315/stock_nxtcmp5_partition_sampled_baseline_gt-only	
% /Users/jteoh/Code/BigFuzz/hybridfuzz/evaluation_logs_20220315/stock_nxtcmp5_partition_sampled_phased_gt-only
\begin{tabular}{| c || r | r |}
\cellcolor{black}{\textcolor{white}{\at{\bf Fuzzing\ Step}}}
& \cellcolor{black}{\textcolor{white}{\at{\bf Duration\ (ms)}}}
&\cellcolor{black}{\textcolor{white}{\at{\bf \#Iterations}}}
\\\hline
\hspace{-1ex}
Intermediate Seed Computation & 1450 & -
\\\hline
UDF Fuzzing & 205084 & 4775
\\\hline
Inverse Function Application & 601 & -
\\\hline
\makecell{End-to-end Fuzzing with\\ Improved Seed (\tool)} & 208 & 1
\\\hline
\tool Total & 207346 & -
\\\hline
Baseline & 14401113 & 40010*
\\\hline
\end{tabular}
